Near-Optimality for Single-Source Personalized PageRank

The \emph{Single-Source Personalized PageRank} (SSPPR) query is central to graph OLAP, measuring the probability $\pi(s,t)$ that an $\alpha$-decay random walk from node $s$ terminates at $t$. Despite decades of research, a significant gap remains between upper and lower bounds for its computational complexity. Existing upper bounds are $O\left(\min\left(\frac{\log(1/\epsilon)}{\epsilon^2}, \frac{\sqrt{m \log n}}{\epsilon}, m \log \frac{1}{\epsilon}\right)\right)$ for SSPPR-A and $O\left(\min\left(\frac{\log(1/n)}{\delta}, \sqrt{m \log(n/\delta)}, m \log \left(\frac{\log(n)}{m\delta}\right)\right)\right)$ for SSPPR-R, with trivial lower bounds of $\Omega(\min(n,1/\epsilon))$ and $\Omega(\min(n,1/\delta))$. This work narrows or closes this gap. We improve the upper bounds for SSPPR-A and SSPPR-R to $O\left(\frac{1}{\epsilon^2}\right)$ and $O\left(\min\left(\frac{\log(1/\delta)}{\delta}, m + n \log(n) \log \left(\frac{\log(n)}{m\delta}\right)\right)\right)$, respectively, offering improvements by factors of $\log(1/\epsilon)$ and $\log\left(\frac{\log(n)}{m\delta}\right)$. On the lower bound side, we establish stronger results: $\Omega(\min(m, 1/\epsilon^2))$ for SSPPR-A and $\Omega(\min(m, \frac{\log(1/\delta)}{\delta}))$ for SSPPR-R, strengthening theoretical foundations. Our upper and lower bounds for SSPPR-R coincide for graphs with $m \in \Omega(n \log^2 n)$ and any threshold $\delta, 1/\delta \in O(\text{poly}(n))$, achieving theoretical optimality in most graph regimes. The SSPPR-A query attains partial optimality for large error thresholds, matching our new lower bound. This is the first optimal result for SSPPR queries. Our techniques generalize to the Single-Target Personalized PageRank (STPPR) query, improving its lower bound from $\Omega(\min(n, 1/\delta))$ to $\Omega(\min(m, \frac{n}{\delta} \log n))$, matching the upper bound and revealing its optimality.

==> floats/algo_balance_X_12.tex <==
\begin{algorithm}[!t]
\caption{BalanceDiff}
\label{algo:balance}
\DontPrintSemicolon
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{
Current $(U,X,Y_1,Y_2)\in \mathcal{U}(n,D,d)$, a sub-graph $G_+\subseteq U$ and initial estimators $\mathsf{ev}_{X_1},\mathsf{ev}_{X_2}$ with $\mathsf{ev}_{X_1}\leq \mathsf{ev}_{X_2}$.
}
\Output{Updated sub-graph $G_+$.}

\If{$\mathsf{ev}_{X_2}\le\mathsf{ev}_{X_1}+nd$}{
  \Return{$G^+$}
}

\For{$i\leftarrow 1$ \KwTo $\lfloor(\mathsf{ev}_{X_2}-\mathsf{ev}_{X_1})/D\rfloor$}{
    Randomly pick a node $x\in\{\,x\in X : \deg_{G_+}(x)\le D/8\}$;\;
    $T_1\leftarrow 0, T_2\leftarrow 0, E_x\leftarrow\varnothing$;;\;
    \For{$j\leftarrow 1$ \KwTo $2D-d$}{
      query $Adj_{in}(x)$ and get the result $(e,y_j)$ with $y_j\notin G_+\cup E_x$;;\;
      $E_x\leftarrow E_x\cup\{(e,y_j)\}$;\;
      \eIf{$y_j\in X_1$}{
        $T_1\leftarrow T_1+1$;\;
      }{
        $T_2\leftarrow T_2+1$;\;
      }
    }
    \If{$T_1 > T_2$}{
    \emph{break}
    }
  %——— 2.3 在 G^+ 中加边 ———
  Randomly select $\tfrac{D}{16}$ edges to $Y_1$ \haoyu{in $D$}{what's the meaning?} and 
  $\tfrac{D}{16}$ edges to $Y_2$ in $D$, add them to $G_+$;\;
}
\Return{$G^+$}
\end{algorithm}


==> floats/algo_bwp.tex <==
\begin{algorithm}[!b]
\caption{Backward Push~\cite{lofgren2014fast} (BP)}
\label{algo:bwp}
\DontPrintSemicolon
  \KwInput{graph $G$, target node $t$, decay factor $\alpha$ and error threshold $r_{max}$.}
  \KwOutput{estimation $\hat{\pi}(t,\cdot)$ and resulted residue $r_t(\cdot)$.}
  $r_t(t)\gets 1;r_t(u)\gets 0$ for all $u \neq t$; \\
  $\hat{\pi}(t,u)\gets 0$ for all $u \in V$;\\
  \While{$\exists u \in V \ s.t.\ r_t(u) \geq r_{max}$}{
  \For{each $v \in N_{in}(u)$}{
    $r_t(v) \gets r_t(v) + (1-\alpha) \cdot r_t(u)/d_{out}(v)$;
    }
    $\hat{\pi}(t,u) \gets \hat{\pi}(t,u) + \alpha \cdot r_t(u);$\\    $r_t(u) \gets 0;$
 }
 \Return{$\hat{\pi}(t,\cdot)$ and $r_t(\cdot)$}
\end{algorithm}

==> floats/algo_enhanced_A.tex <==
\begin{algorithm}[!t]
\label{algo:main}
\caption{$\algo_+$, strengthened algorithm $\algo$.}
\DontPrintSemicolon
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{
Current $(U,X,Y_1,Y_2)\in \mathcal{U}(n,D,d)$, an initial sub-graph $G_+=\varnothing \subseteq U$ and state $\mathcal{S}^{+}=\varnothing.$}
\Output{
  $\mathcal{B}(\mathcal{S}^{+}).$
}
$G\leftarrow \varnothing$,
$S\leftarrow \varnothing$,
$t\leftarrow 0$;\;

\For{$i=1$ \KwTo $nd$}{
    $t\leftarrow t+1$;\;
    $Q_t \leftarrow \algo_+(\mathcal{S}^{+})$;\;
    \If{\haoyu{$Q_t = \mathsf{END}$}{what's $\mathsf{END}$?}}{
        \emph{break}
    }\Else{
        perform query $Q_t$ on $G_+$ and get result $R_t$;\;
        $\mathcal{S}^{+}\leftarrow\mathcal{S}^{+}\cup (Q_t,R_t)$ and $G_+\leftarrow G_+\cup R_t$;\;
        \If{$\bigl|E_{G_+}(Y_1,X)\bigr|>\bigl|E_{G_+}(Y_2,X)\bigr|$}{
        randomly sample a node $y\in Y$ with $\deg^{\mathsf{out}}_{G}(y)<2D-d$;\;
        query $Adj_{out}(y)$ and update $G_+$ with obtained result;
        }
    }
$\mathsf{ev}_{X_1},\mathsf{ev}_{X_1}=EstimateDiff((U,X,Y_1,Y_2), G_+)$;\;
$G_+=BalanceDiff\left((U,X,Y_1,Y_2), G_+, \mathsf{ev}_{X_1}, \mathsf{ev}_{X_2}\right)$;
}
\Return{$\mathcal{B}(\mathcal{S}^{+}).$}
\end{algorithm}


==> floats/algo_estimate_X_12.tex <==
\begin{algorithm}[!t]
\caption{EstimateDiff}
\label{algo:estimate}
\DontPrintSemicolon
\KwInput{Current $(U,X,Y_1,Y_2)\in \mathcal{U}(n,D,d)$ and a sub-graph $G_+\subseteq U.$}
\KwOutput{Edge estimators $\mathsf{ev}_{X_1},\mathsf{ev}_{X_2}$.}
% initializations
$\mathsf{ev}_{X_1}\!\leftarrow 0$, $\mathsf{ev}_{X_2}\!\leftarrow 0$ and $\mathsf{FAC}\;\leftarrow\;\bigl|E_{G_+}(X_1\cup X_2,\;X)\bigr|/\bigl\lfloor nd/D\bigr\rfloor$;\\
% main loop
\For{$i\leftarrow 1$ \KwTo $\bigl\lfloor nd/D\bigr\rfloor$}{
  % sample one across‐cut edge
  Uniformly sample an edge $(y,x)$ from $E_{G_+}(X_1\cup X_2,\;X)$\;
  $D_1\leftarrow 0$, $D_2\leftarrow 0$\;
  % examine D incoming neighbors of x
  \For{$j\leftarrow 1$ \KwTo $D$}{
    query $Adj_{in}(x)$ and get the result $(e,y_j)$\;
    \eIf{$y_j\in X_1$}{
      $D_1\leftarrow D_1+1$\;
    }{
      $D_2\leftarrow D_2+1$\;
    }
  }
  % accumulate to whichever side is heavier
  \eIf{$D_1>D_2$}{
    $\mathsf{ev}_{X_1}\leftarrow \mathsf{ev}_{X_1} + \mathsf{FAC}$\;
  }{
    $\mathsf{ev}_{X_2}\leftarrow \mathsf{ev}_{X_2} + \mathsf{FAC}$\;
  }
}
\Return{$\mathsf{ev}_{X_1},\;\mathsf{ev}_{X_2}$}
\end{algorithm}


==> floats/algo_fwp.tex <==
\begin{algorithm}[!b]
\caption{Forward Push~\cite{sp} (FP)}
\label{algo:fwp}
\DontPrintSemicolon
  \KwInput{graph $G$, source node $s$, decay factor $\alpha$ and error threshold $r_{max}$.}
  \KwOutput{estimation $\hat{\pi}(s,\cdot)$ and resulted residue $r_s(\cdot)$.}
  $r_s(s)\gets 1;r_s(u)\gets 0$ for all $u\neq s$; \\
  $\hat{\pi}(s,u)\gets 0$ for all $u \in V$;\\
  \While{$\exists u \in V \ s.t.\ r_s(u) \geq r_{max}/d_{out}(u)$}{
  \For{each $v \in N_{out}(u)$}{
    $r_s(v)\gets r_s(v) + (1-\alpha) \cdot r_s(u)/d_{out}(u)$;
    }
    $\hat{\pi}(s,u)\gets \hat{\pi}(s,u) + \alpha \cdot r_s(u);$\\    $r_s(u)\gets 0;$
 }
 \Return{$\hat{\pi}(s,\cdot)$ and $r_s(\cdot)$}
\end{algorithm}

==> floats/algo_pwp.tex <==
\begin{algorithm}[!t]
\caption{Power Push (PP, simplified~\cite{wu2021unifying} with equivalent theoretical property)}
\label{algo:pwp}
\DontPrintSemicolon
  \KwInput{graph $G$, source node $s$, decay factor $\alpha$ and error threshold $r_{max}$.}
  \KwOutput{estimation $\hat{\pi}(s,\cdot)$ and resulted residue $r(\cdot)$.}
  $r(s,s)\gets 1;r(s,u)\gets 0$ for all $u\neq s$; \\
  $\hat{\pi}(s,u)\gets 0$ for all $u \in V$;\\
  initialize a \textit{first-in-first-out} queue $Q \gets \{u\}$;\\
  \While{$Q \neq \emptyset \text{ and } r_{sum}> r_{max}\cdot m$}{
    $v \gets Q.\text{pop}();$\\
    $\hat{\pi}(s, v) \gets \hat{\pi}(s, v) + \alpha \cdot r(s, v);$\\
    \For{\textbf{each} $u \in N_\text{out}(v)$}
        {$r(s, u) \gets r(s, u) + \frac{(1 - \alpha) \cdot r(s, v)}{d_v}$;\\
        if $u \notin Q$ and $r(s,u)\geq r_{max}$, $Q.\text{append}(u);$\\}
    $r(s, v) \gets 0$;
    }
    Repeat lines $3-6$ in Algorithm~\ref{algo:spush}.
\end{algorithm}

==> floats/fig_gb_instance.tex <==
\begin{figure}[!h]
\centering
% \vspace{-0.6cm}
\includegraphics[width=0.36\textwidth]{figs/fig_Gb_instance.jpg}
% \vspace{-0.3cm}
\caption{An example for generating graph distribution $\mathcal{G}(D,\mathbf{b})$.} %\haoyu{modify the graph.}
\label{fig:gb_instance}
\end{figure}

\begin{comment}

\begin{wrapfigure}{l}{0.29\textwidth} % r/l for side; set box width
  \vspace{-\intextsep} % optional: tighten vertical gap
  \centering
  \includegraphics[width=\linewidth]{figs/fig_Gb_instance.jpg}
  \vspace{-1.8\intextsep}
  \caption{Example of $\mathcal{G}(D,\mathbf{b})$.}
  \label{fig:gb_instance}
  \vspace{-\intextsep}
\end{wrapfigure}

\end{comment}

==> floats/fig_new_hard_instance.tex <==
%\begin{figure}[!t]
%\includegraphics[width=0.47\textwidth]{figs/fig_new_hard_instance.png}
%\centering
%\caption{Graph instance family $\mathcal{U}(n, D, d)=\mathcal{U}(3, 2, 1)$.} 
%\label{fig:instance}
%\vspace{-0.5ex}
%\end{figure}


\begin{wrapfigure}{l}{0.47\textwidth}
  \includegraphics[width=\linewidth]{figs/fig_new_hard_instance.png}
  \vspace{-3\intextsep}
  \caption{Instance family $\mathcal{U}(n, D, d)=\mathcal{U}(3, 2, 1)$.}
  \vspace{-\intextsep}
  \label{fig:instance}
\end{wrapfigure}

==> floats/fig_path_decom.tex <==
%\begin{figure}[!b]
%\includegraphics[width=0.4\textwidth]{figs/fig_path_decom.jpg}
%\centering
%\caption{Illustration of our decomposition of a single path} 
%\label{fig:path_decom}
%\vspace{-0.5ex}
%\end{figure}

\begin{wrapfigure}{l}{0.42\textwidth}
  \vspace{-2em}
  \centering
  \includegraphics[width=0.4\textwidth]{figs/fig_path_decom.jpg}
  \vspace{-2em}
  \caption{Decomposition of a single path.}
  \label{fig:path_decom}
  
\end{wrapfigure}


==> floats/fig_ur_1_instance.tex <==
\begin{wrapfigure}{l}{0.29\textwidth} % r/l for side; set box width
  \vspace{-\intextsep} % optional: tighten vertical gap with surrounding text
  \centering
  \includegraphics[width=\linewidth]{figs/fig_Ur_1_instance.jpg}
  \vspace{-1.5\intextsep}
  \caption{Instance $\mathcal{U}^{-1}(r)$}
  \label{fig:u-1_instance}
  \vspace{-\intextsep}
\end{wrapfigure}
\begin{comment}
\begin{figure}[!h]
\centering
%\vspace{-0.6cm}
\includegraphics[width=0.5\textwidth]{figs/fig_Ur_1_instance.jpg}
%\vspace{-0.3cm}
\caption{Instance $\mathcal{U}^{-1}(r)$}
\label{fig:u-1_instance}
\end{figure}
\end{comment}

==> floats/notation.tex <==
\begin{table}[ht]
\centering
\color{black}
\setlength{\abovecaptionskip}{0.5mm}
\setlength{\belowcaptionskip}{0.5mm}
\caption{Frequently used notations in this paper.}
\label{tab:fre_notations}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{p{.25\textwidth}| p{.7\textwidth}}
\toprule
    \textbf{Notations} & \textbf{Descriptions}\\
    \midrule
    
    $HARD(n, m, \Delta, \gamma)$ & a distribution of directed graph\\\hline
    
    $n ,m, \Delta, \gamma$ & 
    parameters of $HARD$ i.e. 
    each graph in $HARD$ has $\Theta(n)$ nodes, $\Theta(m)$ edges, $\Delta = \Theta(\frac{1}{\delta}), \gamma = \Theta(1)$ \\\hline
    
    $X_1, X_2, Y_1, Y_2, Z, s $  & subgraph of $HARD$ \\\hline
    
    
    $Q$ & a query in some query model\\\hline
    
    $H, U$ & a instance in $HARD$, or covered subgraph after a sequence of queries\\\hline
    

    % parameters used in the proof details

    $E_{H}(V, W)$ & the set of edges from $V$ to $W$ in graph $H$\\\hline
    
    $deg_{H}(x, W), deg_{H}(W, x)$ & the number of edges from $x$ to $W$ or from $W$ to $x$  in graph $H$\\\hline
    
    $\mathcal{M}, \cost(A,x), ver(A, x)$ & family of deterministic algorithms, the function of cost and verification of result \\\hline
    
    $RAND(\mathcal{M})$ & distributions (randomized algorithms) over $\mathcal{M}$\\\hline
    
    $\varphi, C,\,p$ & map function, cost blow‑up and success‑loss parameters in simulations\\\hline
    
    $\widetilde{HARD}$ & a larger family of directed graph allowing parallel edges\\\hline
    $HARD(U), \widetilde{HARD}(U)$ & a subfamily of graphs \\ \hline
    
    $\mathfrak{G}, \mathfrak{G}(U)$ & the symmetry group of $\widetilde{HARD}$ and stablizer subgroup for covered fixed subgraph\\
    
    \bottomrule
\end{tabular}
\end{table}

==> floats/tab_best_known_old.tex <==
\begin{table}[!t]
\caption{Best-Known results and our Improvements of SSPPR-A, SSPPR-R and STPPR query. We highlight our new results in \textcolor{red}{red} and bold the \textbf{Improvements} when $\epsilon, \delta$ are sufficiently small. For ease of simplicity, we here assume the number of edges, $m\in \bigo(n^{2-\beta})$ for any given arbitrary small constant $\beta\in(0,1)$ in our Tighter SSPPR-A Lower Bounds.}

%\footnote{We found that the concurrent work~\cite{bertram2025estimating}, independently draw new lower bound on single node PPR with relative error of $\Omega(\min(m,\frac{1}{\delta}))$ and STPPR of $\Omega(\min(m,\frac{n}{\delta}))$.}
%Note that~\cite{bertram2025estimating} is a recent concurrent work to ours, and we remark its results with \underline{underlining}. We also highlight our \textbf{improvement} when $\epsilon, \delta$ are sufficiently small. For ease of simplicity, we here assume $m\in \bigo(n^{2-\beta})$ for any arbitrary small constant $\beta\in(0,1)$ in our Tighter SSPPR-A lower bound.}
\centering
\label{tab:pprs}
\renewcommand{\arraystretch}{3.0}
%\setlength{\tabcolsep}{18pt}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{|c|c|c|c|}
\toprule
 & \textbf{Best-Known Lower Bounds} & \textbf{Tighter Lower Bounds\footnote{123}} & \textbf{Improvements} \\
\midrule
SSPPR-A & $\Omega\left(\min(n, \frac{1}{\epsilon})\right)$~\cite{wei2024approximating} & {\color{red}$\Omega\left(\min(m, \frac{1}{\epsilon^2})\right)$} & $\frac{1}{\epsilon}$ or ${\frac{m}{n}}$ \\ \hline
SSPPR-R & $\Omega\left(\min(n, \frac{1}{\delta})\right)$~[\textcolor{myblue}{TRIVIAL}] & {\color{red}$\Omega\left(\min(m, \frac{\log(\frac{1}{\delta})}{\delta})\right)$} & $\log(\frac{1}{\delta})$ or ${\frac{m}{n}}$\\ \hline
STPPR & $\Omega\left(\min(n, \frac{1}{\delta})\right)$~\cite{rbs} & {\color{red}$\Omega\left(\min(m, \frac{n}{\delta}\log(n))\right)$} & $n\log(n)$% , \textcolor{red}{[Optimal]}\\
\\ \midrule
  & \multicolumn{3}{c|}{\textbf{Best-Known (\textcolor{red}{Improved}) Upper Bounds}} \\
\midrule
STPPR & \multicolumn{3}{c|}{$\bigo\left(\min(m\log(\frac{1}{\delta}), \frac{n}{\delta}\cdot\log(n))\right)$} %matches our lower bound of {\color{red}$\Omega\left(\min(m, \frac{n}{\delta}\log(\frac{1}{\delta}))\right)$}}\
\\\hline
SSPPR-R & \multicolumn{3}{c|}{$\bigo\left(\min(\frac{\log(1/\delta)}{\delta}~\text{\cite{mc}}, \sqrt{\frac{m \log(n)}{\delta}}~\text{\cite{fora}}, m \log\left(\frac{\log(n)}{\delta m}\right)~\text{\cite{wu2021unifying}})\right)$} \\ \hline
\multirow{2}{*}{SSPPR-A} & \multicolumn{3}{c|}{$\bigo\left(\min(\frac{\log(1/\epsilon)}{\epsilon^2}~\text{\cite{mc}}, \frac{\sqrt{m \log(n)}}{\epsilon}~\text{\cite{wei2024approximating}}, m \log\frac{1}{\epsilon}~\text{\cite{wu2021unifying}})\right)$} \\ 
&\multicolumn{3}{c|}{$\to\bigo\left(\min({\color{red}\frac{1}{\epsilon^2}~[\text{Ours}]}, \frac{\sqrt{m \log(n)}}{\epsilon}~\text{\cite{wei2024approximating}}, m \log\frac{1}{\epsilon}~\text{\cite{wu2021unifying}})\right)$}\\
\bottomrule
\end{tabular}}
\end{table}



==> floats/tab_notations_twopages.tex <==
\begin{table}[ht]
    \caption{Notations and Descriptions (Part 1 of 2)}
    \label{tab:notations_part1}
    \centering
    \renewcommand{\arraystretch}{1.2} 
    \begin{tabularx}{\textwidth}{p{2.8cm} X}
        \toprule
        \textbf{Notation} & \textbf{Description} \\
        \midrule
        
        % --- SECTION 1: Graph Basics ---
        $G = (V_G, E_E)$ & Underlying directed graph with node set $V$, edge set $E$; or simply $(V, E)$ \\
        
        $n, m$ & Number of nodes, edges in $G$ \\
        
        $\alpha$ & Constant decay factor defining PageRank and PPR; $\alpha \in (0, 1)$\\

        $p$ & Constant failure probability bound\\
        
        $\delta, c$ & Relative error setting threshold; constant relative error parameter \\
        
        $\epsilon$ & Absolute error setting parameter \\
        
        $\pi(s, t),\pi_G(s,t)$ & Personalized PageRank scores between nodes $s, t$ in $G$\\

        \query{ADJ}, \query{DEG}, \query{JUMP} & Queries in arc-centric model\\

        \midrule 
        
        % --- SECTION 2: Graph Properties ---
        $e = (u, v)$ & Directed edge from node $u$ to $v$ \\
        
        $d_{out}^G(u), d_{in}^G(u)$ & Out-degree, in-degree of node $u$ in $G$ \\

        $V_{\ge \delta}, X_{\geq \delta}$ & Subset of $V$ with PPR scores $\ge \delta$\\

        $V_{\mathrm{out}}, X_{\mathrm{out}}$ & Candidate node set output by algorithm \algoa\\

        $\overleftrightarrow{p_G}(u,v)$ & Set of all directed paths between node pair $(u,v)$ in $G$\\
        
        $\footnotesize\overleftrightarrow{p}, w_G({\footnotesize\overleftrightarrow{p}})$ & Path in $G$; path weight regarding $\alpha$-decay random walk\\

        $\boundary{X}$ & Nodes in $V \setminus X$ having out-edge to set $X$\\

        \midrule

        % --- SECTION 3: Weights and Sums (Start) ---
        $\mathbf{{S}_r}(u)$ & Weight in Lemma \ref{lemma:newdecom}; $\mathbf{{S}_r}(u)=\frac{1}{\alpha}{{\pi}_G(s,u)d_{\mathrm{out}}^{G_X}(u)}/{d_{\mathrm{out}}^{G}(u)}$\\

        $\hat\pi_G(s,v)$ & Estimated PPR scores\\

        $\mathbf{{\hat S}_r}(u)$ & Empirical weight in Lemma \ref{lemma:newdecom}; $\mathbf{{\hat S}_r}(u)= \frac{1}{\alpha}{\hat{\pi}_G(s,u)d_{\mathrm{out}}^{G_X}(u)}/{d_{\mathrm{out}}^{G}(u)}$\\

        $\texttt{SUM}(\mathbf{\hat{S}_r}) $ & Total score summation; $\texttt{SUM}(\mathbf{\hat{S}_r}) = \sum_{u\in\boundary{X}}\mathbf{{\hat S}_r}(u) $\\

        $\mathbf{\hat{\bar{S}}_r}$ & Normalized weight distribution; $\mathbf{\hat{\bar{S}}_r}:=\mathbf{\hat{S}_r}/\texttt{SUM}(\mathbf{\hat{S}_r})$\\
        
        \bottomrule
    \end{tabularx}
\end{table}

\begin{table}[ht]
    \caption{Notations and Descriptions (Part 2 of 2)}
    \label{tab:notations_part2}
    \centering
    \renewcommand{\arraystretch}{1.2} 
    \begin{tabularx}{\textwidth}{p{2.8cm} X}
        \toprule
        \textbf{Notation} & \textbf{Description} \\
        \midrule

        % --- SECTION 3: Weights and Sums (Continued) ---
        $c_r, p_r,\delta_r$ & Parameters in Algorithm \algorr\\

        $N_r, H[v]$ & Total walk count in \algorr; walks ending at node $v$\\

        $X_r$ & Remaining target (non-estimated) subset after round $r$\\
        
        $V_r$ & Newly estimated subset in round $r$; $V_r = X_{r-1} \setminus X_r$\\

        $R$ & Round bound in \algor; last execution round if context clear\\

        $\Delta$ & Constant shrink factor in \algor; $\Delta>1$\\

        \midrule

        % --- SECTION 4: Hard Instances ---
        $ \mathcal{U}(n, D, d)$ & Hard-instance multigraph family with parameters $D, d$\\

        $\mathrm{U}, \mathrm{U}(r)$ & (Multi)graph in family $ \mathcal{U}(n, D, d)$; its $r$-padded instance\\

        $\Sigma(n, D, d)$ & Distribution over family $ \mathcal{U}$ \\

        $\mathrm{SP}\in \binom{X}{2}$ & Split of set $X$ into $X_1, X_2$; generator part for $\Sigma(n, D, d)$\\

        $\mathrm{MUL}(\mathrm{U})$ & Edge multiplicity of multigraph $\mathrm{U}$ (Def. \ref{def:multigraph})\\ 

        $\mathcal{A}_{(\cdot)}$ & Algorithms in Lemmas \ref{lemma:algo_lift}, \ref{lemma:res_algo}, \ref{thm:algo_adapt_tot} \\

        $e_t$ & Event in $\Sigma(n, D, d)$: $k^{\text{th}}$ out-edge of $y_i$ connects to $k'^{\text{th}}$ in-edge of $x_j$\\

        \midrule
        
        % --- SECTION 5: Appendix / Advanced ---
        $\tau$ & Constant for geometric sequence $\delta_0, \delta_0\tau, \delta_0\tau^2, \dots$ (Appendix ~\ref{sec:adaptive_thre})\\

        $K_{\mathrm{RW}}, K_{\mathrm{err}}, K_{\mathrm{prob}}$ & Constants in \newalgor{} related to $N_r, c_r, p_r$\\

        $\mathbf{1}_A$ & Indicator function of event $A$\\
        
        $\mathrm{All}_{r-1}$ & Random variable for information available before round~$r$ estimation\\
        
        $ \hat\pi_G^{(r)}(s,t)$ & Estimate of $\pi_G(s,t)$ based on prior estimates (Eq. ~\eqref{eq:def_coherent_estimation})\\

        $D_r(t)$ & Martingale-difference sequence of estimation error at node $t$(Eq. ~\eqref{eq:def_diff_free})\\
        
        \bottomrule
    \end{tabularx}
\end{table}

==> floats/tab_uppersotas.tex <==
\begin{table}[!b]
\caption{Upper Bounds of SSPPR-R query.}
\centering
\label{tab:pprs}
\renewcommand{\arraystretch}{1.2}
%\setlength{\tabcolsep}{18pt}
%\resizebox{0.6\textwidth}{!}{
\begin{tabular}{c|c}
\toprule
\textbf{Technique\haoyu{replace with two tables the other for lower bound}}  & \textbf{Complexity} \\
\midrule
MC~\cite{mc} &  $\bigo\left(\frac{\log\left(n\right)}{\delta}\right)$ \\ \hline
FORA~\cite{fora} &  $\bigo\left(\sqrt{\frac{m\log\left(n\right)}{\delta}}\right)$ \\ \hline
SpeedPPR~\cite{wu2021unifying} &  $\bigo\left(m\log\left(\frac{\log\left(n\right)}{\delta m}\right)\right)$\\ 
\bottomrule
\end{tabular}
%}
\end{table}


==> text/construction.tex <==
\newpage
\section{Proof Framework: Lower Bound of SSPPR-R}
\label{sec:proof}
In this section, we present the proof framework for deriving Theorem~\ref{thm:ssppr-r}. We couple the proof details of Theorem~\ref{thm:ssppr-a} as they share similar hard instance structure. We begin bt first introducing the high-level ideas.

\paragraph{High-Level Ideas.}
We begin by constructing a carefully designed graph instance family, denoted by $\mathcal{U}(n, D, d)$, parameterized by integers $n$, $D$, and $d$ to be specified later. Each instance $\mathrm{U} \in \mathcal{U}(n, D, d)$ contains a distinguished \emph{source} node $s$ and $2n$ \emph{target} nodes, evenly partitioned into two disjoint sets: $X_1$ and $X_2$, as illustrated in Figure~\ref{fig:U_instance}. By carefully engineering the edge structure, we ensure that every node $x_1 \in X_1$ has a higher PPR value from $s$ than any node $x_2 \in X_2$, satisfying $\pi(s,x_1) - \pi(s,x_2) \geq 2\varepsilon$ for SSPPR-A, or $\pi(s,x_1)/\pi(s,x_2) \geq 2/(1 - c)$ for SSPPR-R, as shown in Lemmas~\ref{lemma:PPR_A} and~\ref{lemma:PPR_R}, respectively. That is, nodes in $X_1$ and $X_2$ differ in their PPR values by at least the required additive or relative error threshold. To succeed in this setting, any algorithm $\algo$ must detect structural differences between nodes in $X_1$ and $X_2$, which are intentionally subtle and primarily reflected in degree statistics. To model this formally, we define a uniform distribution $\Sigma(n, D, d)$ over the legal graph instances, as described in Lemma~\ref{lemma:legal_instance}. This distribution is constructed by considering all valid permutations of node and edge labels and all balanced splits of the $X$ node set. Under this formulation, we can quantify the success probability of any algorithm $\algo$ operating under a query budget $T$. A subtle technical challenge arises from the potential presence of \emph{parallel edges}, which may occur in our multigraph construction. Lemma~\ref{lemma:paraBoundU} guarantees that the maximum multiplicity of parallel edges is bounded by a constant $L$ with high probability. Combined with Theorem~\ref{thm:multiedge}, this ensures that any algorithm $\algo$ designed for simple graphs can be adapted to work on multigraphs without incurring significant additional query complexity.

Bringing these components together, we establish Theorem~\ref{thm:AtoU}, which asserts that if the query budget falls below a certain threshold—specifically, {\small$T = o\left(\min(m, \frac{\log(1/\delta)}{\delta})\right)$} for the SSPPR-R problem—then no algorithm $\algo$ can correctly recover the $X_1$–$X_2$ split with constant probability. Indeed, Lemma~\ref{lemma:targetProb} shows that under such constraints, the expected success probability is upper-bounded by $1/n$. As a result, any algorithm that satisfies the SSPPR query guarantees must make at least {\small$\Omega\left(\min(m, \frac{\log(1/\delta)}{\delta})\right)$} queries. This completes the proof of the lower bounds stated in Theorems~\ref{thm:ssppr-r}.% and~\ref{thm:ssppr-a}.


%Theorem~\ref{thm:main} asserts that any such $\algo$ cannot achieve this distinguishing task with constant probability if its overall expected query cost is bounded by $o\bigl(\frac{\log(1/\varepsilon)}{\varepsilon}\bigr)$, thereby establishing the main lower bound.

%To prove this theorem, we employ several key techniques and concepts. First, we transform the notion of \emph{performing queries on a randomly sampled graph from the family} into a \emph{step-by-step} observation of an evolving state.  
%Each state corresponds to a sub-graph composed of the nodes and edges observed so far through the queries executed by the algorithm.  
%This framework enables us to precisely express and tightly bound the success probability of any algorithm \(\algo\) distinguishing \(X_1\) from \(X_2\) by a quantity that decreases polynomially with \(n\), i.e., at most \(\frac{1}{\poly(n)}\).  
%In other words, with probability at least \(1-p\), there exists at least one node in \(X\) that \(\algo\) will misclassify.


%A key subtlety arises because real algorithms may adaptively choose queries based on the history of observed states. To address this, we ensure that the family $\mathcal{U}$ remains indistinguishable under automorphisms even with a small allowance for parallel edges, enabling simulation of any algorithm on “simple” graphs with minimal additional cost. Furthermore, we introduce \emph{balanced querying}, augmenting adaptive algorithms with dummy queries to reduce dependency on past observations and maintain analytical tractability. Finally, we reduce the adaptive process to a sequence of approximately independent experiments, allowing application of classical lower bound techniques to the adaptive setting.

\input{floats/fig_hard_instances}

% \paragraph{Remark.} Throughout this paper, for technical soundness, we assume  
% $\min\!\left(m, \frac{1}{\delta} \log \frac{1}{\delta}\right) = \mathcal{O}\bigl(n^{2-\beta}\bigr)$
% for some constant $\beta > 0$.

\subsection{Hard Instance Family --- $\mathcal{U}(n,D,d)$}
We define the graph family $\mathcal{U}(n, D, d)$ such that, for every sufficiently large $n$, it serves as a collection of hard instances for estimating SSPPR queries. This family is constructed based on a simple yet insightful core structure $\mathbf{U}$, illustrated in Figure~\ref{fig:U_instance}. The graph consists of five disjoint node sets: $\{s\} \cup Y_1 \cup Y_2 \cup X_1 \cup X_2$. For brevity, we let $Y = Y_1 \cup Y_2$ and $X = X_1 \cup X_2$. The node $s$ serves as the designated \emph{source} node, while all nodes in $X$ act as \emph{target} nodes whose PPR values with respect to $s$ are of interest. We ensure that each of the sets $X_1$, $X_2$, $Y_1$, and $Y_2$ contains $\Theta(n)$ nodes. Regarding edge construction, each node $y_1 \in Y_1$ receives an incoming edge from the source node $s$. For each node $x_1 \in X_1$, we construct $D$ incoming edges from nodes in $Y_1$ (i.e., $\deg_{Y_1}(x_1) = D$) and $D - d$ edges from $Y_2$ (i.e., $\deg_{Y_2}(x_1) = D - d$). Similarly, each $x_2 \in X_2$ receives $D$ edges from $Y_2$ and $D - d$ from $Y_1$. The critical difference is that nodes in $X_1$ are indirectly reachable from $s$ via a \emph{useful} path through $Y_1$, whereas nodes in $X_2$ are only connected through \emph{useless} paths via $Y_2$ that do not connect to $s$. This design ensures a measurable PPR gap between $X_1$ and $X_2$. Additionally, we impose that every node $y \in Y$ has out-degree $d_{\text{out}}(y) = 2D - d$ to ensure uniformity and support our lower-bound construction. With appropriately chosen parameters, we show that nodes in $X_1$ and $X_2$ exhibit a clear and quantifiable difference in their PPR values with respect to $s$. This distinction is formally captured in Lemma~\ref{lemma:PPR_A} for the SSPPR-A query and in Lemma~\ref{lemma:PPR_R} for the SSPPR-R query. To facilitate analysis in the SSPPR-R setting, we next introduce a modified structure, referred to as the $r$-padded instance, which better accommodates the relative-error guarantees.

\begin{definition}[$r$-padded instance] 
 \(\forall\mathrm{U} \in \mathcal{U}(n, D, d)\), we define the \emph{\(r\)-padded} instance of \(\mathrm{U}\), denoted as \(\mathrm{U}(r)=(V_{U(r)},E_{U(r)})\) in the below by involving two independent node sets $Z_X$ and $Z_Y$:
\begin{enumerate}
    \item $V_{U(r)}=V_U\cup Z_X\cup Z_Y$, where $Z_X,Z_Y$ are two additional node sets containing exactly $r$ nodes;
    \item $E_{U(r)}=E_U \cup \{(z_x, x)\;\mid \forall x \in X, z_x \in Z_X\} \cup \{(y, z_y)\;\mid \forall y \in Y, z_y \in Z_Y\}$, which incorporates extra edges coming from node set $Z_x$ to $X$ and $Y$ to $Z_Y$.
\end{enumerate}
\end{definition}
An illustrative example is provided in Figure~\ref{fig:U(r)_instance}. The $r$-padded instance $\mathrm{U}(r)$ is specifically designed to facilitate the analysis of SSPPR-R queries. Intuitively, when \(r\) is sufficiently large relative to \(D\), each \query{ADJ} query originating from a node in \(X\) or \(Y\) may be misdirected to the auxiliary node sets \(Z_X\) or \(Z_Y\) with non-negligible probability. This increases the expected query cost for algorithms attempting to explore useful edges. With this construction in place, we now proceed to compute the PPR values from the source node \(s\) to nodes in the sets \(X_1\) and \(X_2\), as formalized in the following lemma:


\begin{lemma}[PPR Calculation]
\label{lemma:PPR_Cal}
For any instance \(\mathrm{U} \in \mathcal{U}(n, D, d)\), the following properties hold:
\begin{enumerate}[label=(\roman*).]
    \item The graph \(\mathrm{U}\) contains \(4n + 1\) nodes and \(2n(2D - d) + n\) edges;
    \item For each node \(x_1 \in X_1\) and \(x_2 \in X_2\), the Personalized PageRank values with respect to the source node \(s\) are
    \(\pi(s,x_1) = (1 - \alpha)^2 \cdot \frac{D}{(2D - d)n}\) and 
    \(\pi(s,x_2) = (1 - \alpha)^2 \cdot \frac{D - d}{(2D - d)n}\).
\end{enumerate}

Moreover, for the \(r\)-padded instance \(\mathrm{U}(r)\) with \(r \geq D\), we have:
\begin{enumerate}[label=(\roman*).]
    \item The graph \(\mathrm{U}(r)\) contains \(4n + 2r + 1\) nodes and \(2n(2D - d + 2r) + n\) edges;
    \item For each node \(x_1 \in X_1\) and \(x_2 \in X_2\), the PPR values are
    \(\pi(s,x_1) = (1 - \alpha)^2 \cdot \frac{D}{(2D - d + r)n}\) and 
    \(\pi(s,x_2) = (1 - \alpha)^2 \cdot \frac{D - d}{(2D - d + r)n}\), 
    and in particular, 
    \(\pi(s,x_2) = \frac{D - d}{D} \cdot \pi(s,x_1)\).
\end{enumerate}
\end{lemma}

\begin{proof}
The number of nodes and edges in both instances $\mathrm{U}$ and $\mathrm{U}(r)$ follows directly from their definitions. We now compute the PPR values from the source node $s$ on the instance $\mathrm{U}$. First, since each node $y \in Y_1$ receives one incoming edge from $s$, and there are $n$ such nodes, it holds that $\pi(s,y) = \frac{1 - \alpha}{n}$. Next, consider nodes $x_1 \in X_1$ and $x_2 \in X_2$. Each node in $X_1$ receives $D$ in-edges from $Y_1$, and each node in $X_2$ receives $D - d$ in-edges from $Y_1$. Since every $y \in Y_1$ has out-degree $2D - d$, the probability of transitioning from a given $y$ to any of its children is $\frac{1}{2D - d}$. By aggregating over all paths from $s$ to $x_1$ via $Y_1$, we obtain
$\pi(s,x_1) = (1 - \alpha)^2 \cdot \frac{D}{(2D - d)n}$ and
$\pi(s,x_2) = (1 - \alpha)^2 \cdot \frac{D - d}{(2D - d)n}$. The difference is then
$\pi(s,x_1) - \pi(s,x_2) = (1 - \alpha)^2 \cdot \frac{d}{(2D - d)n}$. For the padded instance $\mathrm{U}(r)$, the analysis is similar. Each node in $Y$ now has out-degree $2D - d + r$ due to the extra outgoing edges to $Z_Y$. Thus, the transition probabilities are updated accordingly, and we obtain
$\pi(s,x_1) = (1 - \alpha)^2 \cdot \frac{D}{(2D - d + r)n}$ and
$\pi(s,x_2) = (1 - \alpha)^2 \cdot \frac{D - d}{(2D - d + r)n}$. In particular, this yields the ratio $\pi(s,x_2) = \frac{D - d}{D} \cdot \pi(s,x_1)$. This completes the proof.
\end{proof}

Equipped with the above lemma, we now carefully select the graph parameters $n$, $D$, and $d$, along with the error tolerances $\epsilon$ and $\delta$, to ensure that the PPR values of nodes in $X_1$ and $X_2$ exhibit a controlled but noticeable difference.

%\paragraph{Property of graphs in the family}
%\xinpeng{explain these weird conditions are for theoremXXX, switch to \(n_0\)}
\begin{lemma} [SSPPR-A]\label{lemma:PPR_A}
Choose any small constant $\beta \in (0,1)$, decay factor \(\alpha\) and any functions \(\varepsilon_0(n_0)\in (0,1), m_0(n_0)\in\Omega(n_0)\cap \bigo(n^{2-\beta})\). For sufficiently large $n_0$, there exists graph parameters \(n, D, d\) (as function of \(n_0\)) s.t. for all graph instance $\mathrm{U} \in \mathcal{U}(n,D,d)$, the following conditions hold:

\begin{enumerate}[label=(\roman*).]
\item The node count of \(\mathrm{U}\) is in $\bigo(n_0)$, and the edge count \(\mathrm{U}\) is in $\bigo(m_0)$;
\item \((n)^{1-\beta} \geq D\geq 2d\) and \(d\leq\log(n)\);
\item \(Dn \ \text{is } \Omega\left(\min( m_0, \frac{\log(\frac{1}{\varepsilon_0})}{\varepsilon_0})\right)\);
\item For all node $x_1\in X_1$ and $x_2\in X_2$, their PPR values satisfy $$\pi(s,x_1)-\pi(s,x_2) > 2\varepsilon_0.$$
\end{enumerate}
\end{lemma}

\begin{proof}

We manipulate the parameters \(n\) and \(D\) to fulfill the conclusion. Let \(C\) be a constant to be determined later. We set 
\(n D = C \beta^2 \min\left(n_0^{2-\beta}, m_0, \frac{\log(1/\varepsilon_0)}{\varepsilon_0}\right)\), \(n \geq D\), and \(d = \log(n)\). Note that \(d \geq \frac{1}{2} \log(n D)\). From Lemma~\ref{lemma:PPR_Cal}, we have:
\begin{align*}
\pi(s,x_1) - \pi(s,x_2)&=\frac{d}{2D - d} \cdot \frac{(1 - \alpha)^2}{n} \geq \frac{\log(nD)}{8Dn} \cdot (1 - \alpha)^2\geq \frac{\log(C\beta^2\frac{\log(\frac{1}{\varepsilon_0})}{\varepsilon_0})}{8C\beta^2\frac{\log(\frac{1}{\varepsilon_0})}{\varepsilon_0}}  \cdot (1 - \alpha)^2\\
& \geq \frac{(1-\alpha)^2}{8C\beta^2}  \frac{\log(\frac{1}{\varepsilon_0}) + log(C\beta^2) + \log\log(\frac{1}{\varepsilon_0}) }{\log(\frac{1}{\varepsilon_0})}\varepsilon_0 \geq \frac{(1-\alpha)^2}{16C\beta^2} \varepsilon_0
\end{align*}
The last inequality requires \(\log(C\beta) + \log(\frac{1}{\varepsilon_0}) > \frac{1}{2}\log(\frac{1}{\varepsilon_0})\), which further needs $\varepsilon_0<(C\beta)^{2}$. Setting $C=\Theta((1-\alpha)^2)$ directly accomplishes the property $(iv)$. Next, we need to fit the conditions $(i), (ii)$ and $(iii)$ to accomplish the proof. We give an overall setting of 
$$
n = \left( C\beta^2 \min(n_0^{2-\beta}, m_0, \log(\frac{1}{\varepsilon_0})/{\varepsilon_0})\right)^{\frac{1}{2-\beta}}\ \text{and}\ D = \left(  C\beta^2 \min(n_0^{2-\beta}, m_0, \log(\frac{1}{\varepsilon_0})/{\varepsilon_0})\right)^{\frac{1-\beta}{2-\beta}}. 
$$
Condition $(i)$ holds since the total number of edges is at most \(2n(2D - d) + n \leq 4n D = \Theta(\beta m_0)\), and the number of nodes is \(4n + 1 = \Theta(\beta n_0)\). For condition~(ii), it is clear that \(n^{1 - \beta} \geq D\), and since \(2d = 2 \log n \leq \log\left((C \beta^2)^{2/(2 - \beta)} n_0\right)\), we have \(2d \leq (C \beta^2 n_0)^{(1 - \beta)/(2 - \beta)} \leq D\) for sufficiently large \(n\). Finally, condition $(iii)$ holds directly by the definition of \(n D\).
% and thus we finish the proof.
\end{proof}

\begin{lemma}[SSPPR-R]\label{lemma:PPR_R}
Choose any constant \(c\in (0,\frac{1}{2}]\) and any functions \(\varepsilon_0(n_0)\in (0,1), m_0(n_0)\in\Omega(n_0)\cap \bigo(n^{2})\). For sufficiently large $n_0$, there exists graph parameters \(n, D, d, r\)  (as function of \(n_0\)), such that for $r$-padded instance $\mathrm{U}(r)$ based on all graph instance $\mathrm{U} \in \mathcal{U}(n,D,d)$, following conditions hold:
\begin{enumerate}[label=(\roman*).]
    \item The node count of \(\mathrm{U}(r)\) is in $\bigo(n_0)$, and the edge count \(\mathrm{U}(r)\) is in $\bigo(m_0)$;
    \item \((n)^{\frac{1}{2}} > D\geq \frac{3}{2}d\) and \(d\leq \log(n)\);
    \item \(n(r+D) =  \Omega\left(\min(m, \frac{\log(\frac{1}{\delta_0})}{\delta_0})\right)\);
    \item For all $x_1\in X_1$ and $x_2\in X_2$ with PPR values satisfying $\pi(s,x_1)\geq \delta_0$ and $\pi(s,x_2)\geq \delta_0$, we have $$\pi(s,x_1) \geq \frac{1}{(1-c)^2}\cdot \pi(s,x_2).$$
\end{enumerate}
\end{lemma}
\begin{proof}
We consider two cases with an overall setting of $\delta$ such that 
$\frac{\log\frac{1}{\delta}}{\delta} = \min(c m_0, \frac{\log\frac{1}{\delta_0}}{\delta_0}).$
\paragraph{Case 1:} $
n_0 \leq \frac{1}{32} (1-\alpha)^2 \frac{1}{\delta}.$ And we here set $n = n_0, \quad d = \log(n_0), \quad D = \left(1 + \frac{1}{4c}\right) d$ and $ r = \frac{(1-\alpha)^2d}{16 c n_0 \delta} > 0.$
Under these parameters, conditions (i), (ii), and (iii) naturally hold when $n$ is sufficiently large. Moreover for condition (iv), we have
\[
n r = \Omega\left((1-\alpha)^2 d/\delta c\right) = \Omega\left( \min(m_0, \frac{\log\frac{1}{\delta_0}}{\delta_0})\right).
\]
By Lemma~\ref{lemma:PPR_Cal}, the PPR value for any $x_2 \in X_2$ satisfies
\[
\pi(s,x_2) = (1-\alpha)^2 \frac{D - d}{(2D - d + r) n_0} 
= \frac{(1-\alpha)^2}{(4c + 2) n_0 + \frac{(1-\alpha)^2}{4 \delta}} \geq \delta \geq \delta_0.
\]
\paragraph{Case 2:}  $n_0 > \frac{1}{32} (1-\alpha)^2 \frac{1}{\delta}.$ Under this setting, we set $r = 0$ since 
no padded instance is required here. Further, we give $n = \frac{1}{32} (1-\alpha)^2 \frac{1}{\delta}$ and $ D = \left(1 + \frac{1}{4c}\right) d.$ Similarly, for sufficiently large $n$, conditions (i), (ii), and (iii) hold. Additionally, it holds that $n D = n d \left(1 + \frac{1}{4c}\right) = \Omega\left(\frac{\log(\frac{1}{\delta})}{\delta} \right)=\Omega\left( \min(m_0, \frac{\log\frac{1}{\delta_0}}{\delta_0})\right)
$ and $\pi(s,x_2) = \frac{(1-\alpha)^2}{n (4c + 2)} \geq \delta \geq \delta_0$, which ensures condition (iv) and thus we complete the proof. 
\end{proof}

Lemma~\ref{lemma:PPR_A} shows that the node sets $X_1$ and $X_2$ differ in their PPR values by more than twice the error parameter $\varepsilon_0$. Consequently, any algorithm $\algo$ must distinguish between these two sets with constant success probability, otherwise we argue that it is impossible to distinguish the two node sets with expected query cost at $o(\frac{\log(1/\varepsilon_0)}{\varepsilon_0})$ in later sections. 

Notice that under the assumption \(\min(m_0, \frac{\log(1/\varepsilon_0)}{\varepsilon_0}) \leq n_0^{2-\beta}\), the instance family we construct contains \(nD = \Theta\left(\min(m_0, \frac{\log(1/\varepsilon_0)}{\varepsilon_0})\right)\) edges, which is proportional to the total query complexity stated in Theorem~\ref{thm:ssppr-a}. To prove this main theorem, it suffices to show that there exists an absolute constant \(C_A\) such that any algorithm attempting to solve the SSPPR-A problem with expected query cost at most \(C_A \cdot (1 - p)nD\) must fail on our constructed graph family with probability at least \(p\). By Markov's inequality, we can enforce that the algorithm halts and raises an error if it performs more than \(C_A \cdot \frac{nD}{\beta}\) queries, and subsequently demonstrate the existence of a graph instance on which the failure probability is at least \(\frac{p}{2}\).

A similar argument applies in the SSPPR-R setting, where the expected query budget is bounded by \(C_R \cdot nD\) for some constant \(C_R\). To derive these conclusions, we first formalize the execution of a specific query \(Q\) and its corresponding response \(R\) as an \emph{event} on an instance \(\mathrm{U} \in \mathcal{U}(n, D, d)\) with assigned node and edge labels.




==> text/morebounds.tex <==
\section{Update}

\subsection{Concentration Inequalities}
Throughout this section, we use the following well-known Chernoff bounds.
\begin{theorem}[Chernoff]
Let \(X_1,\ldots,X_n\) be independent random variables taking values in \([0,1]\). Let \(X := \sum_{i=1}^n X_i\) and \(\mu := \mathbb{E}[X]\). Then, for any \(c>0\),
\begin{enumerate}
    \item if \(c\in[0,1]\), then \(\Pr[X > (1+c)\mu] \le \exp\!\big(-\tfrac{c^2}{3}\mu\big)\);
    \item if \(c\in[0,1]\), then \(\Pr[X < (1-c)\mu] \le \exp\!\big(-\tfrac{c^2}{2}\mu\big)\);
    \item if \(c\ge 1\), then \(\Pr[X > (1+c)\mu] \le \exp\!\big(-\tfrac{c}{3}\mu\big)\).
\end{enumerate}
\end{theorem}
\subsection{Revisiting Monte Carlo Estimator}
Although our main contribution is a lower bound, in this section we present a brief refinement of upper bounds to close the gap. The standard Monte Carlo estimator~\cite{mc} is designed to provide uniform accuracy guarantees across all \(n\) nodes. This uniformity naturally introduces a \(\log n\) factor in the complexity.

This approach is well suited to regimes requiring very high precision (e.g., thresholds on the order of \(1/n\)). However, it is overly conservative when the target precision is more moderate. Our main lower bound captures this dependence on the precision parameter: for any threshold \(\delta\), in the single-source relative-error setting we show a bound of \(\Omega\!\big(\min\{m,\, \log(1/\delta)/\delta\}\big)\). Motivated by this, we introduce a more refined two-phase estimator.

In the first (discovery) phase, we execute a collection of random walks to identify a candidate set of nodes whose PPR likely exceeds the threshold. In the second (estimation) phase, we allocate effort only to nodes within this candidate set and estimate their PPR more carefully.

By decoupling discovery from estimation, we avoid the need for uniform guarantees over all \(n\) nodes. Consequently, the \(\log n\) term in the complexity is replaced by a logarithmic dependence on the size of the discovered set from the first phase.

We now focus on the first phase. The goal of the algorithm is to output a subset satisfying:
\begin{enumerate}[label=(\roman*)]
\item \textbf{(No false negatives).} For every \(u\in V\) with \(\pi(s,u)\ge \delta\), we have \(u\in R_\text{out}\).
\item \textbf{(No false positives, margin \(\tfrac{1}{5e}\)).} For every \(u\in R_\text{out}\), \(\pi(s,u)\ge \tfrac{1}{5e}\,\delta\).
\end{enumerate}
We implement this via a two-round filtering. In Round~1 we execute \(\alpha\)-decay random walks and discard every node that never appears as an endpoint. In Round~2 we execute additional walks and discard nodes whose counts fall below a threshold.
\\[-1ex]
\input{floats/algo_discovery}
Should I explain these magic numbers?

For notational convenience, let \(V_{\ge \tau}:= \{\, v\in V : \pi(s,v)\ge \tau \,\}\). Since \(\sum_{v}\pi(s,v)=1\), we have \(|V_{\ge \tau}|\leq 1/\tau\).

\begin{lemma}[Discovering nodes of interest]\label{lemma:discover}
Algorithm \ref{algo:discover} using \(\bigo(\frac{\log\frac{1}\delta}{\delta})\) queries in the standard arc-centric models. It returns, with probability at least \(1-p\), a subset \(R_{\text{out}}\) such that \(V_{\geq \delta} \subseteq R_{\text{out}} \subseteq V_{\geq \delta/(5e)}\).
\end{lemma}

\begin{proof}
Let \(L := \left\lceil \ln \tfrac{1}{\delta}+\ln \tfrac{2}{p} \right\rceil\). The parameters are set to \(T_1 = L\lceil\frac{1}{\delta}\rceil\), \(T_2 = 20L\lceil\frac{1}{\delta}\rceil\), and \(\theta = 10L\). We bound three failure events, aiming for a failure probability of at most \(p/2\), \(p/4\), and \(p/4\) respectively.

\textbf{i. (No false negatives in Round 1).}
Fix \(u \in V_{\ge\delta}\). Since \(T_1 \ge L/\delta\), the probability that \(u\) is never an endpoint in \(T_1\) walks is
\[
\Pr[u \notin R^{\rm raw}_{\text{out}}] = (1 - \pi(s,u))^{T_1} \le (1-\delta)^{T_1} \le e^{-\delta T_1} \le e^{-L} = \delta \frac{p}{2}.
\]
A union bound over all \(u \in V_{\ge\delta}\), where \(|V_{\ge\delta}|\le 1/\delta\), gives a total failure probability for this event of \(\Pr[V_{\ge\delta}\not\subseteq R^{\rm raw}_{\text{out}}]\le \frac{1}{\delta} \cdot \delta \frac{p}{2} = \frac{p}{2}\).

\textbf{ii. (No false negatives in Round 2).}
For any \(u\in V_{\ge\delta}\), the expected count is \(\mu_u := \mathbb{E}[H[u]] = T_2 \pi(s,u) \ge 20L\lceil\frac{1}{\delta}\rceil\delta \ge 20L\). We test if the count \(H[u]\) falls below \(\theta=10L\). Since \(\theta \le \mu_u/2\), we can use the second Chernoff bound with \(c=1/2\):
\[
\Pr[H[u]<\theta] \le \Pr[H[u] < \mu_u/2] \le \exp(-\mu_u/8) \le e^{-20L/8}=e^{-2.5L}=\left(\delta\tfrac{p}{2}\right)^{2.5}.
\]
A union bound over \(u\in V_{\ge\delta}\) gives a total failure probability of
\(\Pr[\exists u\in V_{\ge\delta}:H[u]<\theta]\le \frac{1}{\delta} \cdot \left(\delta\tfrac{p}{2}\right)^{2.5} = \delta^{1.5}(\tfrac{p}{2})^{2.5}\), which is less than \(p/4\) for \(\delta\le 1/2\).

\textbf{iii. (No false positives in Round 2).}
Consider a node \(u\) with \(\pi(s,u) < \delta/(5e)\). Its expected count is \(\mu_u = T_2\pi(s,u) < 20L\lceil\frac{1}{\delta}\rceil \frac{\delta}{5e} = \frac{4L}{e}\delta\lceil\frac{1}{\delta}\rceil\). Using the strict inequality \(\delta\lceil 1/\delta \rceil < 1+\delta\), for \(\delta \le 1/2\) we have \(\mu_u < \frac{4L}{e}(1.5) = \frac{6L}{e}\). We test if \(H[u]\) exceeds \(\theta=10L\). We set \(c=\theta/\mu_u-1 > \frac{10L}{6L/e}-1 = \frac{5e}{3}-1 > 3.5 > 1\). Using the third Chernoff bound,
\[
\Pr[H[u]\ge \theta] \le \exp\!\big(-\tfrac{\theta-\mu_u}{3}\big) < \exp\!\big(-\tfrac{L(10-6/e)}{3}\big) < e^{-2.5L}=\left(\delta\tfrac{p}{2}\right)^{2.5}.
\]
The set of candidates from the first round, \(R^{\rm raw}_{\text{out}}\), has size at most \(T_1\). A union bound over these candidates gives a total failure probability of
\[
\Pr\big[\exists u\notin V_{\ge \delta/(5e)}: u\in R_{\text{out}}\big]
\le T_1 \cdot e^{-2.5L}
\le L(\tfrac{1}{\delta}+1) \left(\delta\tfrac{p}{2}\right)^{2.5}
< p/4
\]
for \(\delta\le 1/2\) and sufficiently small \(p\). A final union bound over the three events yields a total failure probability of at most \(p/2+p/4+p/4 = p\).
\end{proof}

We now design the second phase in each error model. The single-source relative-error case follows directly.

\begin{lemma}
The single-source personalized PageRank problem with a relative-error guarantee can be solved within expected \(O\!\big(\tfrac{\log(1/\delta)}{\delta}\big)\) queries in the standard arc-centric query model.
\end{lemma}

\begin{proof}
By Lemma~\ref{lemma:discover}, using \(O(\log(1/\delta)/\delta)\) random walks (of constant expected length) we obtain \(R_{\text{out}}\) with
\(V_{\ge \delta} \subset R_{\text{out}} \subset V_{\ge \delta/(5e)}\) with failure probability at most \(p/2\).
Then perform
\[
T \;=\; 256\,\frac{\log\!\big(\tfrac{1}{\delta/(5e)}\big)+\log\!\big(\tfrac{2}{p}\big)}{c^2\,(\delta/(5e))}
\;=\; O\!\big(\tfrac{\log(1/\delta)}{\delta}\big)
\]
independent \(\alpha\)-decay random walks from \(s\). As in the standard estimator, for each \(u\in R_{\text{out}}\) estimate \(\pi(s,u)\) by the empirical hit frequency. By Chernoff and a union bound over \(|R_{\text{out}}|\le |V_{\ge \delta/(5e)}|\le 5e/\delta\), the additional failure probability is at most \(p/2\). Nodes outside \(R_{\text{out}}\) are reported as \(0\).
\end{proof}

For the single-source absolute-error case, Lemma~\ref{lemma:discover} remains useful: we can output \(0\) for nodes outside \(V_{\ge \frac{\varepsilon}{5e}}\). Under \(C_1/\varepsilon^2\) random walks, the failure probability at a node \(u\) is bounded by a Chernoff tail of the form \(\exp(-\Omega(\pi(s,u)\cdot C_1/\varepsilon^2))\) when the target absolute tolerance is at most a constant multiple of \(\pi(s,u)\). The subtlety arises when \(\pi(s,u)\ll \varepsilon\), since Chernoff requires the tolerance to be smaller than the mean. Our preprocessing ensures we only estimate nodes in \(R_{\text{out}}\subseteq V_{\ge \varepsilon/(5e)}\), and we tighten the tolerance to \((\varepsilon/(5e))/4\); this incurs only a constant-factor overhead while enabling a direct Chernoff application.

\begin{lemma}
The single-source personalized PageRank problem with an absolute-error guarantee can be solved within expected \(O(1/\varepsilon^2)\) queries in the standard arc-centric query model.
\end{lemma}

\begin{proof}
First obtain \(R_{\text{out}}\) with
\(V_{\ge \varepsilon} \subset R_{\text{out}} \subset V_{\ge \varepsilon/(5e)}\) with failure probability at most \(p/2\) (Lemma~\ref{lemma:discover}). Then execute
\[
T \;=\; 1024\,\frac{\log\!\big(\tfrac{2}{p}\big)}{\big(\tfrac{\varepsilon}{5e}\big)^2}
\;=\; O\!\big(\tfrac{1}{\varepsilon^2}\big)
\]
independent \(\alpha\)-decay random walks from \(s\), and estimate \(\pi(s,u)\) for \(u\in R_{\text{out}}\) by the empirical frequency with tolerance \(\varepsilon/5e\).

Because the new absolute tolerance is not greater than the PPR value for all \(u\in R_{\text{out}}\), the tolerance is not greater than the mean for "the count as endpoint". Chernoff yields
\[
\Pr\!\left[\text{fail at }u\right]
\;\le\; 2\exp\!\left(-\tfrac{1}{3}\,\pi(s,u)\cdot
\Big(\tfrac{\tfrac{\varepsilon}{5e}}{\pi(s,u)}\Big)^2 \cdot T\right)
\;\le\; 2\exp\!\left(-\ln\tfrac{2}{p} - \tfrac{1}{\pi(s,u)}\right)
\;=\; p \, e^{-1/\pi(s,u)}
\;\le\; \tfrac{p}{2}\,\pi(s,u),
\]
where the last inequality uses \(e^{-1/x}\le x/2\) for all \(x\in(0,1]\) (absorbed into the constant in \(T\)). Summing over \(u\) and using \(\sum_u \pi(s,u)=1\) gives a total failure probability at most \(p/2\). Together with the discovery phase, the overall failure probability is at most \(p\).
\end{proof}

\subsection{Lower bounds for other cases}

Though in most of the setting of single target personalized pagerank computation, the optimized algorithm's complexity does not contain a log term. The case "single target personalized pagerank with relative error guarantee" has a trivial upperbound by Monte-Carlo method: \(O(n\log(n)\delta^{-1})\). In this setting, our method still apply and show that this trivial method is already optimal. The tricky point is in this setting, we cannot replace \(\log(n)\) with \(\log(\delta^{-1})\).

\begin{lemma} (STPPR-R)\label{lemma:TPPR}
we use \(\mathrm{U}^{-1}\) for the inverse graph of a graph \(\mathrm{U}\) i.e. reversing the direction of each edge. Choose any decay factor \(\alpha\), error parameter \(c\leq \frac{1}{2}\), and any functions \(\delta_0(n_0)\in (0,\frac{(1-\alpha)^2}{16}), m_0(n_0)\in\Omega(n_0)\cap \bigo(n^2_0)\). For sufficiently large $n_0$, there exists graph parameters \(n, D, d\) (as function of \(n_0\)) s.t. for all graph instance $\mathrm{U} \in \mathcal{U}(n,D,d)$, the following conditions hold for \(\mathrm{U}^{-1}\).  

\begin{enumerate}[label=(\roman*).]
\item The node count of \(\mathrm{U}\) is in $\bigo(n_0)$, and the edge count \(\mathrm{U}\) is in $\bigo(m_0)$;
\item \((n)^{\frac{1}{2}} \geq D\geq 2d\) and \(d\leq\log(n)\);
\item \(Dn \ \text{is } \Omega\left(\min( m_0,n_0\log(n_0)\frac{1}{\delta_0})\right)\);
\item For all $x_1\in X_1$ and $x_2\in X_2$ with PPR values satisfying $\pi(x_1,s)\geq \delta_0$ and $\pi(x_2, s)\geq \delta_0$, we have $$\pi(x_1,s) \geq \frac{1}{(1-c)^2}\cdot \pi(x_2, s).$$
\end{enumerate}
\end{lemma}
\begin{proof}
Like in the original setting, in \(\mathrm{U}^{-1}\) for $x_i\in X_1$ , \(\pi(x_i, s) = (1-\alpha)^2\frac{D}{2D-d+r}\);  for $x_{i'}\in X_1$ , \(\pi(x_{i'}, s) = (1-\alpha)^2\frac{D-d}{2D-d+r}\). Their fraction is still \(\frac{D-d}{D}\).
In the case \(m_0 >n_0\log(n_0)\frac{1}{\delta_0}\). We can set \(n = n_0, d = \log(n_0), D = \left(1 + \frac{1}{4c}\right) d, r = d(\frac{(1-\alpha)^2}{4c\delta_0} - 1 - \frac{1}{4c})\). The edge count is in \(O(n(D+r)) = O(n_0\log(n_0)\frac{1}{\delta_0}) \subset O(m)\); node count is in \(O(max(n, r)) = O(max(n, m/n)) = O(n)\). As for ppr, \(\pi(x_2, s)\) for \(x_2 \in X_2\) is just \(\delta_0\). And the fraction meets the requirement similarly as in Lemma\ref{lemma:PPR_R} \\ \

Another case is \(\frac{1}{\delta_0} \leq m_0 < n_0\log(n_0)\frac{1}{\delta_0}\). By continuity, there are positive numbers \(n, \delta\),  s.t. \(n \log(n) \frac{1}{\delta} = m\) and \(n \leq n, \delta \geq \delta_0, \binom{n}{2}\geq m\). We also set \(d = log(n),  D = \left(1 + \frac{1}{4c}\right) d, r = d(\frac{(1-\alpha)^2}{4c\delta} - 1 - \frac{1}{4c})\). Then \(\pi(x_2, s) = \delta \geq \delta_0\). Also \(n(r+D) \in \Omega(\frac{nd}{\delta}) = \Omega(m)\); the edge count is in \(O(n(r+D)) = O(\frac{nd}{\delta}) = O(m)\); the node count is \(O(max(n, r)) = O(n, m/n) \subset O(n_0)\),
\end{proof}


As in Theorem \ref{thm:main}, to estimate $\pi(x_i, s)$, one needs the exact split of $X$ into $X_1$ and $X_2$. Since in arc-centric query model a graph and its inverse are the same, we can apply Lemma \ref{lemma:targetProb} to $\mathrm{U} \in \mathcal{U}(n,D,d)^{-1}$, which yields that STPPR-R requires $\Omega\left(\min( m_0,n_0\log(n_0)\frac{1}{\delta_0})\right)$ oracle queries.

\section{Draft for single source absolute case}
\(D^2 =  N=\Theta(1/\varepsilon^2), T = o(N)\)

\(V = \{s\} \cup \{t\} \cup X \cup Y \cup X' \cup Y', |X| = ... = D\), in \(G_0\), \(X,Y\) is fully connected; similarly for \(X', Y'\).
Given a \(N\) bit boolean sequence \(b_1,..., b_N\), each \(k \in \{1,...,N\}\) corresponds to a pair \((i, j) \in  \{1,...,D\} \times  \{1,...,D\} \).  We can define \(G(b_1b_2...b_N)\) by swapping the edge \((x_i, y_j), (x_i', y_j')\) for each \(b_{(i,j)} = 0\).


Pick \(B_i \sim Bern(1/2)\) i.i.d., and \(S:= \sum B_i\), we know that \((1-\alpha)^3 - \pi(s,t) = \Theta(S\varepsilon^2) \) . To calculate \(\pi(s,t)\) with absolute error requires \(\Omega(N)\) queries. 

\(\mu = N/2, \sigma = \sqrt{N}/4\), \(\sigma^{-1}(S-\mu) \text{ tends to } \mathcal{N}(0,1)\). 
Now we go into the event \(Q_1=R_1,...,Q_T=R_T\), conditioned on \(S=k\). Denote the founded swapped edges count as \(l\), then \(P[Q_1=R_1,...,Q_T=R_T|S=s] \sim \text{Hypergeom}(N, s, T)\). Then we have \((S-L)|_{L=l} \sim\text{Binomial}(N-T, 1/2)\), a standard Central limit theorem for binomial, we know that for whatever function \(f, \Pr[|S-f(l)|_{l}>c\sqrt{N}] \in \Theta(1)\), which means the guess of \(\pi(s,t)\) always has a gap of \(\Omega(\varepsilon)\).

\input{text/ssppr_a_lower}

\section{An concern in rebuttal}
A natural question arises: while we have shown that Pr[most likely outcome | sequence of events] is low, one might be concerned about the dependency between the events $Q_1 = R_1, \ldots, Q_T = R_T$ and the algorithm itself, where $R_t$ represents the result of query $Q_t$. Does this algorithmic dependency invalidate our analysis?

This concern can be addressed through the following formal result:

\begin{lemma}
Consider a collection of events $E_0, E_1, \ldots, E_n$ such that for any subset $S \subseteq \{1, \ldots, n\}$ with $|S| \leq m$, we have
$$\Pr\left[E_0 \mid \bigwedge_{s \in S} E_s\right] \in \left(\frac{1}{2} - \varepsilon, \frac{1}{2} + \varepsilon\right).$$

Let $\mathcal{A}$ be any algorithm that operates as follows: at each step $t \leq T < m$, it selects a subset $S_t \subset \{1, \ldots, n\}$ such that the events $\{E_s : s \in S_t\}$ are mutually disjoint (regardless of whether we condition on $E_0$ or $\neg E_0$). The algorithm's choices may depend on the outcomes of previous steps and the joint distribution of $E_0, \ldots, E_n$. After $T$ steps, $\mathcal{A}$ outputs a prediction for $E_0$.

Then $\Pr[\mathcal{A} \text{ succeeds}] \leq \frac{1}{2} + \varepsilon$.

\end{lemma}
This follows directly from the data processing inequality. Regardless of the strategy employed by the algorithm, it cannot extract more information about $E_0$ from the observed events than what is inherently contained in those events themselves.

The key insight is that algorithmic adaptivity does not circumvent fundamental information-theoretic limitations: no computational procedure can amplify the predictive signal beyond what the underlying data structure permits.

==> text/rebuttal.tex <==



\section{Review 2}
Thank you for the comment. Although the numerical gain is modest in some regimes, our main contribution is narrowing the longstanding gap between sub-linear lower bounds and near-linear upper bounds for small $\delta$. Moving from  $\tilde O(m)$ to $\tilde O(n) + O(m)$ demonstrates that the lower bounds obtained via graph query models are indeed representative of the problem's inherent complexity, justifying their use in this context.








==> text/relatedwork.tex <==
\section{Other Related Works}
\label{sec:related_work}
Over the past decades, Personalized PageRank (PPR) computation has been extensively studied, with most research focusing on accelerating and scaling single-source~\cite{mc,fora,wu2021unifying,luo2019baton,yoon2018tpa,avrachenkov2007monte,lrh2022efficient,lrh2023efficient,liu2016powerwalk}, single-target~\cite{lofgren2013personalized,lofgren2015bidirectional,wang2016hubppr,rbs,setpush}, and top-$k$~\cite{fujiwara2012fast,lofgren2015bidirectional,lofgren2014fast,fora,topppr} queries on general graphs.  
Early methods such as~\cite{avrachenkov2007monte,mc,liu2016powerwalk,fujiwara2012fast} employed large-scale Monte Carlo (MC) simulations to estimate PPR values, whereas~\cite{lofgren2013personalized,andersen2006local} applied deterministic graph traversal to compute exact vectors.  
Subsequent algorithms~\cite{fora,wu2021unifying,luo2019baton,topppr,lofgren2015bidirectional,wang2016hubppr} improved scalability by combining deterministic traversal and MC in separate phases.  
More recent approaches~\cite{rbs,setpush,rbs_simrank} integrate deterministic traversal and MC in a unified \emph{Randomized Push} (RS) framework; while RS can answer SSPPR-R queries, it requires $\bigo(\log^3 n/\delta)$ time~\cite{liu2024bird}, worse than basic MC, and is therefore omitted in many practical comparisons.  
Other lines of work study PPR in dynamic graphs~\cite{ohsaka2015efficient,mo2021agenda,hou2023personalized,li2023zebra,zhu2024personalized} and its coupling with graph neural networks~\cite{scara,scara_j,sigma}. Despite this rich algorithmic progress, the \emph{theoretical landscape}—in particular, tight upper and lower bounds for single-source absolute (SSPPR-A), single-source relative (SSPPR-R), and single-target (STPPR) queries—remains underdeveloped.  
The main obstacle is the lack of hard instances specifically tailored to single-source computation, which makes proving lower bounds much more challenging.  
Our work addresses this gap by providing new, significantly tighter lower bounds and a novel proof framework, thereby deepening the theoretical understanding of PPR query complexity and offering fresh directions for future research.

==> text/ssppr_r_lower.tex <==
\input{text/construction}

\paragraph{Node and Edge Labeling in \(\mathcal{U}(n, D, d)\).}\label{sec:labels}

In accordance with the model specified in Definition~\ref{def:arc-centric}, our graph instances are equipped with both node and edge labels. While our overarching goal is to preserve in-distinguishability among instances within the family, we partially fix the labeling scheme to ensure clarity and consistency throughout the construction process described below:

\begin{enumerate}[label=(\roman*).]
    \item The source node \(s\) is assigned label \(1\);
    \item Nodes in \(X\) are labeled consecutively from \(2\) through \(2n + 1\);
    \item Nodes in \(Y_1\) are labeled from \(2n + 2\) to \(3n + 1\), and nodes in \(Y_2\) from \(3n + 2\) to \(4n + 1\);
    \item The \(i^{\text{th}}\) out-edge of the source node \(s\) points to the node labeled \(2n + 1 + i\).
\end{enumerate}

For ease of reference, we adopt the following conventions in place of explicit numeric labels:
\begin{enumerate}[label=(\roman*).]
    \item \(s\) denotes the node labeled \(1\), which has in-degree zero and out-degree \(n\);
    \item \(x_1, x_2, \ldots, x_{2n}\) refer to the nodes labeled \(2\) through \(2n + 1\), each with in-degree \(2D - d\) and out-degree zero;
    \item \(y_1, y_2, \ldots, y_{2n}\) correspond to the nodes labeled \(2n + 2\) through \(4n + 1\), each with in-degree one and out-degree \(2D - d\);
    \item We use \(y^{(1)}_1, \ldots, y^{(1)}_n\) to refer to nodes \(y_1, \ldots, y_n \in Y_1\), and \(y^{(2)}_1, \ldots, y^{(2)}_n\) for \(y_{n+1}, \ldots, y_{2n} \in Y_2\). For edge references, we denote \((y^{(1)}_i, k)\) as the \(k^{\text{th}}\) out-edge from node \(y^{(1)}_i \in Y_1\), and analogously for nodes in $Y_2$. %\haoyu{$y_{(1,i)}->y^{(1)}_{i}$}
\end{enumerate}

The above notations serve interchangeably to denote both the node label and the corresponding node in the graph. Note that the labeling scheme clearly identifies whether a node belongs to \(Y_1\), \(Y_2\), or \(X\), but it does not distinguish between the subsets \(X_1\) and \(X_2\). Additionally, once a node's label is known, its in-degree and out-degree are assumed to be fully determined. 

We now illustrate how queries operate on a graph \(\mathrm{U} \in \mathcal{U}(n, D, d)\) under this labeling convention. Each query-response pair \((Q, R)\) corresponds to an observable property of \(\mathrm{U}\). For example, consider the node labeled \(x_1 \in X\) and the node labeled \(y^{(1)}_{1} \in Y_1\). Suppose the \(3^{\text{rd}}\) in-edge of \(x_1\) corresponds to the \(2^{\text{nd}}\) out-edge of \(y^{(1)}_{1}\). Then the query \(Q = \query{ADJ}_{\text{in}}(x_1, 3)\) yields the response \(R = (y^{(1)}_{1}, 2)\). Conversely, for any graph \(\mathrm{U}_0 \in \mathcal{U}(n, D, d)\), if executing the query \(Q = \query{ADJ}_{\text{in}}(x_1, 3)\) returns the response \(R = (y^{(1)}_{1}, 2)\), then \(\mathrm{U}_0\) must exhibit exactly this structural property. Under this procedure, any query-response pair \((Q, R)\) is referred to as an \emph{event} with respect to a graph instance distribution, i.e., \(\Sigma(n, D, d)\) (defined later in Section~\ref{sec:distribution}). For any \(\sigma \sim \Sigma(n, D, d)\), it corresponds to a graph \(U_{\sigma}\) with fixed edges and node labels. For brevity, we write such an \emph{event} as \(Q = R\) when the context is clear.


\subsection{Distribution  \(\Sigma(n, D, d)\)}
\label{sec:distribution}
% \haoyu{add some sentence for transition.}
\input{floats/fig_generate_graph}
We now describe the procedure for generating an instance \(\mathrm{U} \in \mathcal{U}(n, D, d)\) with assigned node and edge labels, which together define the distribution \(\Sigma(n, D, d)\) over all possible label permutations. An illustrative example is provided in Figure~\ref{fig:generate graph}. Intuitively, \(\Sigma(n, D, d)\) is constructed by randomly splitting the node set \(X\), thereby determining which node labels in \(X\) belong to \(X_1\) or \(X_2\), and then independently sampling every possible edge permutation that is consistent with the hard-instance template. The complete construction procedure is detailed as follows:


\begin{enumerate}[label=(\roman*).]

    \item \emph{Split of \(X\).} 
    We first choose a split \(\mathrm{SP}\) of the index set \(\{1, \dots, 2n\}\) into two disjoint subsets of size \(n\), which determines the split of the node set \(X\) into \(X_1\) and \(X_2\). Specifically, the nodes labeled \(x_1, \dots, x_{2n}\) are assigned to \(X_1\) or \(X_2\) according to the selected split. We denote the set of all possible such splits by \(\mathrm{SP} \in \binom{X}{n}\). For example, in Figure~\ref{fig:generate graph}, the last column lists nodes \(x_1, \dots, x_4\) (from top to bottom), and the chosen split \(\mathrm{SP} = \{1, 3\}\) assigns nodes labeled \(x_1\) and \(x_3\) to \(X_1\), while nodes \(x_2\) and \(x_4\) belong to \(X_2\);

    \item \emph{Permuting in-edges of nodes in \(X\).}  
    For each node \(x_i \in X\), where \(1 \leq i \leq 2n\), we independently apply a permutation \(\mathrm{P}_i^{2D-d} \in \mathrm{S}^{2D-d}:\{1,\dots,2D - d\}\rightarrow\{1,\dots,2D - d\}\), determining the order of its \(2D - d\) in-edges. These in-edges are then divided into two groups: those coming from \(Y_1\) and those from \(Y_2\). Given the fixed split \(\mathrm{SP}\), if \(x_i \in X_1\), the first \(D\) edges in the permuted order are assigned to originate from nodes in \(Y_1\), and the remaining \(D - d\) edges from \(Y_2\); the assignment is reversed if \(x_i \in X_2\). We denote the space of all such independent permutations over the node set \(X\) as \(\mathrm{S}^{2D - d}(X)\). As illustrated in Figure~\ref{fig:generate graph}, this process is concretely depicted using virtual nodes in the second to fourth columns. Each virtual node in the fourth column represents an in-edge of a corresponding node in \(X\). For example, the fourth virtual node in the fourth column corresponds to the first in-edge of \(x_2\). Applying the permutation \(\mathrm{P}_3 = (1, 3, 2)\), the first and third in-edges of \(x_2\) originate from \(Y_2\) (shown as white-filled nodes), while the second originates from \(Y_1\) (gray-filled);

    \item \emph{Permuting out-edges of nodes in \(Y_1\) and \(Y_2\).} We apply two independent permutations \(\mathrm{P}_{Y_1}^{n(2D - d)}, \mathrm{P}_{Y_2}^{n(2D - d)} \in \mathrm{S}^{n(2D - d)}\) over the set \(\{1, \dots, n(2D - d)\}\) to determine the ordering of the out-edges from nodes in \(Y_1\) and \(Y_2\), respectively. These permutations govern whether the \(k^{\text{th}}\) out-edge of a node \(y^{(1)}_i \in Y_1\) (or \(y^{(2)}_i \in Y_2\)) connects to a node in \(X_1\) or \(X_2\). Specifically, the \(k^{\text{th}}\) out-edge of \(y^{(1)}_i\) points to a node in \(X_1\) if \(\mathrm{P}_{Y_1}^{n(2D - d)}[(2D - d)(i - 1) + k] \leq nD\); otherwise, it connects to a node in \(X_2\). An analogous rule applies for nodes in \(Y_2\) via \(\mathrm{P}_{Y_2}^{n(2D - d)}\). We denote the collections of such permutations as \(\mathrm{S}^{n(2D - d)}(Y_1)\) and \(\mathrm{S}^{n(2D - d)}(Y_2)\), respectively. This step corresponds to determining connections between virtual nodes in the second and third columns of Figure~\ref{fig:generate graph}. For example, if we choose \(\mathrm{P}_{Y_1}^{n(2D - d)} = (1, 3, 2, 4, 5, 6)\), then the first four virtual nodes in the second column represent out-edges connecting to nodes in \(X_1\), as determined by the corresponding permutation values;

    \item \emph{Establishing connections between nodes in \(X\) and \(Y\).}  
    Finally, we determine the actual connections between nodes in \(X\) and \(Y\). Without loss of generality, we describe the connection process for the pair \(X_1\) and \(Y_1\); all other pairs follow analogously by swapping the roles of \(D\) and \(D - d\) and adjusting indices accordingly. We begin by selecting a random bijection \(\mathrm{S}(Y_1, X_1): \{1, \ldots, nD\} \rightarrow \{1, \ldots, nD\}\) to match out-edges of nodes in \(Y_1\) with in-edges of nodes in \(X_1\). (For other pairings, such as \(Y_2\) to \(X_1\), we use a corresponding bijection \(\mathrm{S}(Y_2, X_1)\) over \(\{1, \ldots, n(D-d)\}\).)

    From previous steps, the \(nD\) selected out-edges from \(Y_1\) are encoded as a set of tuples \(\{(y^{(1)}_{i_j}, k_j)\}_{j = 1}^{nD}\), where each tuple represents the \(k_j^{\text{th}}\) out-edge of node \(y^{(1)}_{i_j}\). Likewise, the \(nD\) selected in-edges to \(X_1\) are represented as \(\{(x^{(1)}_{i_j'}, k_j')\}_{j = 1}^{nD}\), with each tuple representing the \(k_j'^{\text{th}}\) in-edge of node \(x^{(1)}_{i_j'}\). Both edge sets are naturally ordered; for instance, each out-edge \((y^{(1)}_{i_j}, k_j)\) can be uniquely indexed by the expression \((2D - d)i_j + k_j\). The bijection \(\mathrm{S}(Y_1, X_1)\) then defines the matching: the \(k_j^{\text{th}}\) out-edge of node \(y^{(1)}_{i_j}\) is connected to the \((k_j')^{\text{th}}\) in-edge of node \(x^{(1)}_{i_j'}\). In Figure~\ref{fig:generate graph}, the mapping \(\mathrm{S}(Y_1, X_1) = (4, 3, 2, 1)\) is visually indicated by edges between the virtual nodes (shown as black-filled) in the third and fourth columns.
\end{enumerate}
By the above construction, we can then derive the following lemmas and definitions, which recover a graph instance $\mathrm{U}\in\mathcal{U}(n, D, d)$ accordingly.

\begin{lemma}
\label{lemma:legal_instance}
For all possible {\small\(\mathrm{SP}, \mathrm{P}_i^{2D-d}, \mathrm{P}_{Y_1}^{n(2D - d)}, \mathrm{P}_{Y_2}^{n(2D - d)}, \mathrm{P} \in \binom{X}{n}\times \mathrm{S}^{2D - d}(X)\times \mathrm{S}^{n(2D - d)}(Y_1)\times\mathrm{S}^{n(2D - d)}(Y_2)\times\Pi_{Y_a\in \{Y_1,Y_2\},X_b\in\{X_1,X_2\}}S(Y_a,X_b)\)}: the above procedure links a legal graph instance \(\mathrm{U}\in\mathcal{U}(n, D, d)\). 
\end{lemma}

\begin{comment}
\begin{lemma}
\label{lemma:legal_instance}
For all possible \(\mathrm{SP}, p_{x_i}, p_{Y_1}, p_{Y_2} \in \binom{X}{n}\times \Pi_{i=1}^{2n}SYM_{in}(x_i) \times SYM_{out}(Y_1) \times SYM_{out}(Y_2) \times \Pi_{a,b\in\{1,2\}}SYM(X_a, Y_b)\): the above procedure links a legal graph instance \(\mathrm{U}\in\mathcal{U}(n, D, d)\). 
\end{lemma} 
\end{comment}
\begin{definition}
\( \Sigma(n, D, d)\) is defined as the uniform distribution over
{\small\(\binom{X}{n}\times \mathrm{S}^{2D - d}(X)\times \mathrm{S}^{n(2D - d)}(Y_1)\times\mathrm{S}^{n(2D - d)}(Y_2)\times\Pi_{Y_i\in \{Y_1,Y_2\},X_i\in\{X_1,X_2\}}S(Y_i,X_i)\)}. For \(\sigma \sim \Sigma(n, D, d)\), we use \(\mathrm{U}_\sigma\) to denote the corresponding labeled graph instance \(\mathrm{U} \in \mathcal{U}(n, D, d)\). For ease of presentation, we write \(\mathrm{U} \sim \Sigma(n, D, d)\) to denote a graph instance sampled from this distribution.
\end{definition}

Based on the above construction and definitions, we now formulate the probability that a graph instance contains parallel edges in the following lemma:
\begin{lemma}%(proof in Appendix~\ref{sec:proof:lemma:paraBoundU})
\label{lemma:paraBoundU}
\(\Pr_{\mathrm{U}\sim \Sigma(n, D, d)}\bigl[\text{edge multiplicity of }\mathrm{U}\geq L\bigr] \leq 4n^2 (\frac{4D}{n})^{L}\), for \(1\leq L\leq D\).
\end{lemma}

Lemma~\ref{lemma:paraBoundU} demonstrates that, with high probability, the edge multiplicity in our constructed graph instances is bounded by a small constant. In other words, high multiplicity edges rarely appear under our construction. Leveraging this result, we show in the next section that any algorithm designed for simple graphs can be adapted to handle multigraphs with bounded edge multiplicity. From Lemmas~\ref{lemma:PPR_R} and~\ref{lemma:PPR_A}, since \(D\) is upper bounded by a sublinear polynomial in \(n\) (see condition~(ii) in both lemmas), we can choose a constant \(L\) such that $$\Pr_{\mathrm{U} \sim \Sigma(n, D, d)}\bigl[\text{edge multiplicity of } \mathrm{U} > L\bigr] \le \frac{1}{n}.$$ In particular, we set \(L = \frac{8}{\beta}\) for the SSPPR-A setting and \(L = 16\) for SSPPR-R.


\subsection{Establishing Main Results}

To prove our main results, such as Theorem~\ref{thm:ssppr-r}, we assume the existence of an algorithm \(\algo\) that successfully answers the SSPPR-R problem with \emph{lower} query complexity than our target lower bound. We then derive a contradiction by showing that the overall success probability over the graph distribution becomes \(\bigo(1/n)\), which violates the requirement of constant success probability. Note that \(\algo\) is designed for simple graphs, whereas instances \( \mathrm{U} \sim \Sigma(n, D, d) \) may admit parallel edges. Fortunately, our earlier analysis guarantees that the edge multiplicity is bounded by a constant with high probability. The following theorem provides a mechanism for executing \(\algo\) on such multigraphs.


%\xinpeng{orinial A0 now A}
\begin{lemma}\label{thm:multiedge}
%(proof in Appendix~\ref{sec:proof:thm:multiedge})
% \input{floats/fig_multiple_edges}
[Reduction from simple to multigraphs]
Choose any constant \(L\), decay factor \(\alpha\in (0,1)\), failure probability \(p\in (0,1)\), constant \(\beta\in(0,1)\), and any function \(\varepsilon(n_0)\in(0,1), m_0(n_0)\in\Omega(n_0)\cap \bigo(n_0^{2-\beta}), T(n_0)>0\) (Or, error bound \(c\in(0,\frac{1}{2}]\), and any function \(\delta(n_0)\in(0,1), m(n_0)\in\Omega(n_0)\cap \bigo(n_0^2)\) for SSPPR-R setting).
Suppose there exists an algorithm \(\algo\) such that, for any simple directed graph with \(\Theta(L n_0)\) nodes and \(\Theta(L n_0 + L m_0)\) edges, \(\algo\) answers the SSPPR-A problem with decay factor $\alpha$, error $\varepsilon$  and failure probability bounded by \(p\) (or SSPPR-R problem with threshold \(\delta\), error bound \(c\)), and expected query complexity $T$ in arc-centric model. 

Then there exists an algorithm \(\algo_L\) in arc-centric model such that, for any integers \(n \leq n_0, \; D,\; d,\; r,\; n(D+r)\leq m\), and any \(\mathrm{U} \in \mathcal{U}(n, D, d)\)  with edge multiplicity bounded by \(L\), \(\algo_L\) solves the SSPPR-A problem with decay factor \(1-(1-\alpha)^3\) and error parameter \(\varepsilon\) (or SSPPR-R problem with threshold \(\delta\), error requirement \(c\)) on \(\mathrm{U}(r)\) for \emph{target} nodes in \(X\), with expected query complexity bounded by a function of \(n_0\) in $\bigo(T)$ and with failure probability bounded by \(p\). Specifically,  \(\mathcal{A}_L\) executes each query \(\query{ADJ}_{in/out}(v, k)\) by a uniformly randomly selection of an uncovered label \(k\) among \(v\)'s in or out edges.
\end{lemma}

Combining all the preceding results, we arrive at the following theorem, which encapsulates the current milestone of our analysis:
%overall proof strategy:

\begin{theorem}\label{thm:AtoU}
Choose any constant \(L\geq \frac{16}{\beta}\) , decay factor \(\alpha\in (0,1)\), failure probability \(p\in (0,1)\), constant \(\beta \in(0,1)\), and any function \(\varepsilon_0(n_0)\in(0,1), m_0(n_0)\in\Omega(n_0)\cap \bigo(n_0^{2-\beta}), T(n_0)=o\left(\min(m_0, \frac{\log(\frac{1}{\varepsilon_0})}{\varepsilon_0})\right)\) (Or, \(L\geq 32\), error bound \(c\in(0,\frac{1}{2}]\), and any function \(\delta_0(n_0)\in(0,1), m_0(n_0)\in\Omega(n_0)\cap \bigo(n_0^2), T(n_0) = o\left(\min(m_0, \frac{\log(\frac{1}{\delta_0})}{\delta_0})\right)\) for SSPPR-R setting). Assume there is an algorithm $\algo$ with failure probability bounded by \(p\), and expected query complexity at \(T\) solves the SSPPR-A problem (or SSPPR-R problem), Then given arbitrary small constant \(\gamma\), when \(n_0\) is sufficiently large, there exists integers \(n\) (sufficiently large)\(,\; D,\; d,\; r\) such that:
\begin{enumerate}[label=(\roman*).]
    \item For any \(\mathrm{U}\in \mathcal{U}(n, D,d)\), \(\mathrm{U}(r)\) contains no more than \(\beta n_0\) nodes and no more than \(\beta m_0\) edges;
    \item \(d\leq \log(n), n\geq 2D, D\geq \frac{3}{2}d\);
\end{enumerate}
And there exists an algorithm \(\mathcal{A}^{'}\) holding that:
\begin{enumerate}[label=(\roman*)., start=3]
    \item \(\mathcal{A}^{'}\) does at most \(T(n_0) \leq \gamma nD\) queries;
    \item For \(\mathrm{U}\sim \Sigma(n, D,d)\), the algorithm \(\mathcal{A}^{'}\) can be applied on any multigraph instance \(\mathrm{U}\), with expected probability at least \(\frac{1-p}{4}\), \(\mathcal{A}^{'}\) can output the correct split \(X_1, X_2\) of \(X\).
\end{enumerate}
\end{theorem}

\begin{proof}
We begin with the SSPPR-R case. For the graph related parameters, Lemma~\ref{lemma:PPR_R} gives the integers \(n,\; D,\; d,\; r\), directly satisfying the condition $(i)$ and $(ii)$ with \(n(D+r) = \Omega\left( \min(m_0, \frac{\log(\frac{1}{\delta})}{\delta_0})\right)\).
Next, we'd construct algorithm $\algo'$ to fit the condition $(iii)$ and $(iv)$. The steps are described as:
\begin{enumerate}[label=(\roman*).]
\item \emph{\(\mathcal{A}\) to \(\mathcal{A}_L\) for executable on multi graph \(\mathrm{U}(r)\)}. As established in our earlier analysis, for \(L = 16\), a graph sampled from the distribution \(\Sigma(n, D, d)\) admits edge multiplicity at most \(L\) with high probability, specifically at least \(1 - \frac{1}{n}\). By invoking Theorem~\ref{thm:multiedge}, this guarantees the existence of an algorithm \(\mathcal{A}_L\) that can solve the SSPPR-R problem on such multigraphs with expected success probability at least \(1 - p\), with expected query complexity of \(o(n(D + r))\).
\item \emph{From PPR estimation to split of \(X\).} To ensure that \(\mathcal{A}_L\) produces PPR estimates of nodes in \(X\) within the specified relative error tolerance \(c\), it must be capable of distinguishing the two subsets \(X_1\) and \(X_2\), whose PPR values differ by a clear, quantifiable gap. We therefore append a simple post-processing step to \(\mathcal{A}_L\) that outputs a split of \(X\) based on the estimated PPR values. This split is correct if the estimates produced by \(\mathcal{A}_L\) satisfy the SSPPR-R accuracy requirements. Specifically, by Lemma~\ref{lemma:PPR_R}, for any \(x_{i_1} \in X_1\) and \(x_{i_2} \in X_2\), we have \(\pi(s,x_{i_1}) \geq \frac{1}{(1 - c)^2} \pi(s,x_{i_2})\). This implies the existence of a threshold \(\pi_0\) such that for all \(x_{i_1} \in X_1\), \(\pi(s,x_{i_1})(1 - c) > \pi_0\), and for all \(x_{i_2} \in X_2\), \(\pi(s,x_{i_2})(1 + c) < \pi_0\). Furthermore, Lemma~\ref{lemma:PPR_R} ensures that \(\pi(s,x_i) \geq \delta\) for all \(x_i \in X\). If \(\mathcal{A}_L\) succeeds on \(\mathrm{U}(r)\), its estimate \(\hat{\pi}(s,x_i)\) must satisfy \(|\hat{\pi}(s,x_i) - \pi(s,x_i)| \leq c \pi(s,x_i)\). As a result, for all \(x_{i_1} \in X_1\), we have \(\hat{\pi}(s,x_{i_1}) \geq (1 - c)\pi(s,x_{i_1}) > \pi_0\), and for all \(x_{i_2} \in X_2\), we have \(\hat{\pi}(s,x_{i_2}) \leq (1 + c)\pi(s,x_{i_2}) < \pi_0\). Thus, \emph{a simple thresholding rule} at \(\pi_0\) suffices to correctly separate \(X\) into \(X_1\) and \(X_2\).
\item \emph{From queries on \(\mathrm{U}(r)\) to queries on \(\mathrm{U}\).} In the previous step, we constructed an algorithm that successfully distinguishes between \(X_1\) and \(X_2\) using an expected \(o(n(D + r))\) queries on the \(r\)-padded graph \(\mathrm{U}(r)\), under the assumption that the edge multiplicity of the underlying graph \(\mathrm{U}\) is bounded by \(L = 16\) with high probability \(1 - \frac{1}{n}\). We now demonstrate that queries involving the auxiliary padding nodes in \(Z_X\) and \(Z_Y\) are not essential. Consequently, the algorithm can be adapted to the original graph \(\mathrm{U}\) with an expected query complexity of \(o(nD)\).

Recall that we have not fixed a specific labeling scheme for \(\mathrm{U}(r)\) in earlier steps; instead, we simply assigned labels to the padding nodes \(Z_X\) and \(Z_Y\) as \(4n + 2,\dots,4n + 2r + 1\). The out-edges from each node \(y_i \in Y\) to \(Z_Y\) are assigned labels \(2D - d + 1,\dots,2D - d + r\), and the in-edges from \(Z_X\) to each \(x_i \in X\) are labeled analogously. Given this fixed labeling, all information regarding \(Z_X\) and \(Z_Y\) is known in advance from the perspective of \(\mathcal{A}_L\). Since \(\mathcal{A}_L\) operates only on \(\mathrm{U}(r)\), these edges can be hard-coded into the algorithm. We initialize a subgraph \(G_0\) internal to \(\mathcal{A}_L\) that stores all such predetermined edges in \(\mathrm{U}(r)\)—specifically, all the nodes \(s\), \(X\), \(Y\), \(Z_X\), and \(Z_Y\), along with the edges from \(Z_X\) to \(X\) and from \(Y\) to \(Z_Y\).

We then define the modified algorithm \(\mathcal{A}'_L\) as follows. The core idea is to simulate \(\mathcal{A}_L\) on the original graph \(\mathrm{U}\) by internally emulating its behavior on the padded graph \(\mathrm{U}(r)\). Whenever \(\mathcal{A}_L\) issues a degree query or an \(\mathsf{Adj}\) query involving a node in the padding sets \(Z_X \cup Z_Y\), \(\mathcal{A}'_L\) returns the predetermined response encoded in \(G_0\), which is consistent across all \(\mathrm{U}(r)\) constructed from some \(\mathrm{U} \in \mathcal{U}(n, D, d)\). In the case where \(\mathcal{A}_L\) issues a query of the form \(\mathsf{Adj}^{\mathrm{in}}(x_i, k)\), we proceed as follows: if \(k > 2D - d\), the query refers to a synthetic edge from \(Z_X\), so we return the \((k - 2D + d + 1)\)-st node in \(Z_X\); otherwise, we forward the actual query \(\mathsf{Adj}^{\mathrm{in}}(x_i, k)\) to the graph \(\mathrm{U}\), and add the resulting edge to the internal subgraph \(G_0\). In this way, \(\mathcal{A}'_L\) simulates the interaction between \(\mathcal{A}_L\) and \(\mathrm{U}(r)\) using queries exclusively on \(\mathrm{U}\). Therefore, with success probability at least \(p\), \(\mathcal{A}'_L\) correctly outputs the split \((X_1, X_2)\).

\item \emph{Bounding query complexity of \(\mathcal{A}_L^{'}\)}. We now bound the query complexity of \(\mathcal{A}'_L\). As described in Theorem~\ref{thm:multiedge}, the algorithm \(\mathcal{A}_L\) issues queries of the form \(\query{ADJ}_{\mathrm{out}/\mathrm{in}}(v, k)\) by selecting \(k\) uniformly at random from the un-queried incident edge labels. For any node \(v \in \mathrm{U}\) where fewer than \((D + r)/2\) incident labels have been examined, the probability that a new query returns a \emph{real} (non-padding) edge is at most \((2D - d)/(2D - d + r - (D + r)/2)\). Consequently, the expected number of genuine adjacency queries issued by \(\mathcal{A}'_L\) can be bounded by the sum of two terms: the first is \((2D - d)\cdot \mathbb{E}[|\{v \in \mathrm{U} \mid \text{at least } (D + r)/2 \text{ incident labels examined}\}|]\); the second is \((2D - d)/(2D - d + r - (D + r)/2)\cdot o((D + r)n)\). Since both terms are asymptotically \(o(nD)\), the overall expected query complexity of \(\mathcal{A}'_L\) is \(o(nD)\).

\end{enumerate}

\end{proof}


For notational simplicity, we refer to the final algorithm constructed in the above theorem as \(\algo\). Naturally, we decompose \(\algo\) into two components: the first part, denoted \(\mathcal{A}_1\), is an \emph{exploration} procedure that performs queries on the graph; the second part, \(\mathcal{A}_2\), processes the information collected and outputs a split of \(X\) into subsets \(X_1\) and \(X_2\). The algorithm \(\algo\) succeeds if and only if \(\mathcal{A}_2\) outputs a correct split. Since we are working under the RAM model, we can assume that \(\mathcal{A}_1\) and \(\mathcal{A}_2\) operate independently—that is, \(\mathcal{A}_2\) is a separate algorithm whose input is the data written into memory by \(\mathcal{A}_1\), and whose output is the inferred split of \(X\). Given that RAM is finite (though arbitrarily large) and that the only inputs to \(\mathcal{A}_1\) are the query responses \(R_1, \ldots, R_T\), we may treat the final RAM state as a function of the query-response sequence \(Q_1, \ldots, Q_T, R_1, \ldots, R_T\), along with any internal randomness. According to the definition in~\ref{df:MAP}, this tuple \((Q_1, \ldots, Q_T, R_1, \ldots, R_T)\) constitutes the \emph{observation}, while the correct split of \(X\) represents the \emph{prior} distribution. The expected success probability of \(\algo\) can thus be formulated as:

\begin{align}
\nonumber
&\mathbb{E}_{\mathrm{U} \sim  \Sigma(n, D, d)}\bigl[\Pr[\algo \text{ succeeds on } U]\bigr]\leq \sum_{Q_1=R_1,\cdots,Q_T=R_T} \Pr_{\algo, {\mathrm{U}\sim \Sigma(n, D, d)}}[Q_1,\cdots,Q_T;R_1,\cdots,R_T] \\
&\times \max_{\mathrm{\mathrm{SP}} \in \binom{X}{n}} \Pr_{\mathcal{U}\sim \Sigma(n, D, d)}[\mathrm{SP} \text{ is the correct split of }  \mathrm{U} \mid Q_1=R_1,\cdots,Q_T=R_T].
\end{align}
Note that the notion of an \emph{event} \(Q = R\) was defined in the final part of Section~\ref{sec:labels}. Our goal now is to evaluate the conditional probability
\[
\Pr_{\mathrm{U} \sim \Sigma(n, D, d)}\left[\mathrm{SP} \text{ is the correct split of } \mathrm{U} \,\middle|\, Q_1, \ldots, Q_T;\, R_1, \ldots, R_T \right],
\]
and to show that it is bounded by \(\frac{1}{n}\). This result is formally captured in the following Lemma~\ref{lemma:targetProb}.

\begin{lemma}
%(proof in Appendix~\ref{sec:proof:lemma:targetProb})
\label{lemma:targetProb}
There is a constant \(\gamma\), such that. For sufficiently large \(n\), \(d \leq log(n)\), \(D>\frac{3d}{2}\),  \(T\leq \gamma nD\). Given any query and returning sequence \(Q_1,\cdots,Q_T;R_1,\cdots,R_T\), and a split of \(X\), \(\mathrm{SP}\) we have:
$$\Pr_{\mathrm{U}\sim \Sigma(n, D, d)}[\mathrm{SP} \text{ is the correct split of }  \mathrm{U} \mid Q_1,\cdots,Q_T;R_1,\cdots,R_T] \leq \frac{1}{n}.$$
\end{lemma}

The intuition for why this lemma holds is that, considering two naive ways of exploring  \(\mathrm{U}\), both require \(\Theta(nD)\) queries to get the correct split: The first way is a traversal of the graph. For instance in a breadth-first search, one need expected \(\Omega(nD)\) queries to get all the information. The second approach is a random walk. For each node \(x\in X\), there are at least \(D-d\) edges from \(Y_1\) to \(X\) and at least \(D-d\) edges from \(Y_2\) to \(x\), the key for determining whether \(x\) is in \(X_1\) or \(X_2\) lies in the left \(d\) edges. Notice that each random walk of length \(1\) from \(X\) has probability at most \(\frac{d}{D}\) to find one these key edges. Assume we have done \(o(D)\) such walks at each point, the probability of finding no key-edges at some node is at least \(n(1 - \frac{d}{D})^{o(D)}\). Since \(d \leq log(n), n(1 - \frac{d}{D})^{o(D)}= \Omega(1)\). Details can be found in Appendix~\ref{sec:proof:lemma:targetProb}. By Lemma~\ref{lemma:targetProb}, we then conclude that the expected success probability of $\algo$ is less than $\frac{1}{n}$ under the total query limits {\small$T\in o\left(\min(m_0, \frac{\log(\frac{1}{\delta_0})}{\delta_0})\right)$} for SSPPR-R problem and {\small$T\in o\left(\min(m_0, \frac{\log(\frac{1}{\varepsilon_0})}{\varepsilon_0})\right)$} for SSPPR-A query. This contradiction illustrates that the assumption in Theorem \ref{thm:AtoU} does not hold. Thus, it requires $\Omega\left(\min(m_0, \frac{\log(\frac{1}{\varepsilon_0})}{\varepsilon_0})\right)$
queries for SSPPR-R and $\Omega\left(\min(m_0, \frac{\log(\frac{1}{\delta_0})}{\delta_0})\right)$ for SSPPR-A problems in expectation, which finally leads to our main lower bound results in Theorem~\ref{thm:ssppr-r}.
